Master equation of discrete time graphon mean field games and teams

In this paper, we present a sequential decomposition algorithm equivalent of Master equation to compute GMFE of GMFG and graphon optimal Markovian policies (GOMPs) of graphon mean field teams (GMFTs). We consider a large population of players sequentially making strategic decisions where the actions of each player affect their neighbors which is captured in a graph, generated by a known graphon. Each player observes a private state and also a common information as a graphon mean-field population state which represents the empirical networked distribution of other players' types. We consider non-stationary population state dynamics and present a novel backward recursive algorithm to compute both GMFE and GOMP that depend on both, a player's private type, and the current (dynamic) population state determined through the graphon. Each step in computing GMFE consists of solving a fixed-point equation, while computing GOMP involves solving for an optimization problem. We provide conditions on model parameters for which there exists such a GMFE. Using this algorithm, we obtain the GMFE and GOMP for a specific security setup in cyber physical systems for different graphons that capture the interactions between the nodes in the system.

==> 3Methodb.tex <==
	\label{sec:methodology}
	In this section, we will provide a backward recursive methodology to compute \glspl{gmfg} for both $\mathbb{G}_{T}$ and $\mathbb{G}_{\infty}$. We will consider Markovian equilibrium strategies of player $\alpha$ which depend on the common information at time $t$, $\mu^G_{t}$, and on its current type $x_t^{\alpha}$.\footnote{Note however, that the unilateral deviations of the player are considered in the space of all strategies.}  Equivalently, player $\alpha$ takes action of the form $A_t^{\alpha}\sim \sigma_t^{\alpha}(\cdot|\mu^G_t,x_t^{\alpha})$. Similar to the common agent approach in~\cite{NaMaTe13}, an alternate and equivalent way of defining the strategies of the players is as follows. We first generate partial function $\gamma_t^{\alpha}:\cX\to\cP(\cA)$ as a function of $\mu^G_t$ through an equilibrium generating function $\theta_t^{\alpha}:\cZ\to(\cX\to\cP(\cA))$ such that $\gamma_t^{\alpha} = \theta_t^{\alpha}[\mu^G_t]$. Then action $A_t^{\alpha}$ is generated by applying this prescription function $\gamma_t^{\alpha}$ on player $\alpha$'s current private information $x_t^{\alpha}$, i.e. $A_t^{\alpha}\sim \gamma_t^{\alpha}(\cdot|x_t^{\alpha})$. Thus $A_t^{\alpha}\sim \sigma_t^{\alpha}(\cdot|\mu^G_{t},x_t^{\alpha}) = \theta_t^{\alpha}[\mu^G_t](\cdot|x_t^{\alpha})$.
	
	For a given prescription function $\gamma^{\alpha}_t = \theta^{\alpha}[\mu^G_t]$, the graphon mean-field $\mu^G_t$ evolves according to the discrete-time McKean Vlasov equation, $\forall y\in\cX$ and $\forall \alpha\in[0,1]$:
	\begin{align}
		\mu^{\alpha}_{t+1}(y) =\sum_{x\in\cX}\sum_{a\in \cA} \mu^{\alpha}_t(x)\gamma^{\alpha}_t(a|x)Q\left(y|x,a,\mu^G_t;g^{\alpha}\right), \label{eq:muG_update}
	\end{align}
	which implies
	\begin{align}
		\mu^{\alpha}_{t+1}&= \phi(\mu^{\alpha}_t,\gamma^{\alpha}_t,\mu^G_t;g^{\alpha})\\
		\mu_{t+1}^G &= \phi(\mu_t^G,\gamma_t;g^{\alpha}) 
	\end{align}

	\subsection{Backward recursive algorithm for $\mathbb{G}_{T}$} \label{sec:fhbr1}
		In this subsection, we will provide a methodology to generate \gmfe of $\mathbb{G}_{T}$ of the form described above. We define an equilibrium generating function $(\theta_t)_{t\in[T]}$, where $\theta_t:\cZ\to\{\cX\to\mathcal{P}(\cA) \}$, where for each $\mu^G_t $, we generate $\tgamma_t = \theta_t[\mu^G_t]$. In addition, we generate a reward-to-go function $(V^{\alpha}_t)_{t\in[T]}$, where $V^{\alpha}_t:\cZ\times\cX\to\mathbb{R}$. These quantities are generated through a fixed-point equation as follows.
		\begin{enumerate}
			\item Initialize $\forall \mu^G_{T+1}, x_{T+1}^{\alpha}\in \cX$,
			\begin{align}
				V^{\alpha}_{T+1}(\mu^G_{T+1},x_{T+1}^{\alpha}) \defeq 0.   \label{eq:VT+1}
			\end{align}

			\item For $t = T,T-1, \ldots 1, \ \forall \mu^G_t$, let $\theta_t[\mu^G_t] $ be generated as follows. Set $\tilde{\gamma}_t = \theta_t[\mu^G_t]$, where $\tilde{\gamma}_t$ is the solution of the following fixed-point equation\footnote{We discuss the existence of solution of this fixed-point equation in Section~\ref{sec:exists}}, $\forall i \in [N],x_t^{\alpha}\in \cX$,
  			\begin{align}
				 \tilde{\gamma}_t(\cdot|x_t^{\alpha}) \in  \arg\max_{\gamma_t(\cdot|x_t^{\alpha})} \E^{\gamma_t(\cdot|x_t^{\alpha})}\left[ R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha})+\delta V^{\alpha}_{t+1}(\phi(\mu^G_t,\tgamma_t;g^{\alpha}), X_{t+1}^{\alpha}) | \mu^G_t,x_t^{\alpha}\right] , \label{eq:m_FP}
			\end{align}
 			where expectation in \eqref{eq:m_FP} is with respect to random variable $(A_t^{\alpha},X_{t+1}^{\alpha})$ through the probability measure $\gamma_t(a_t^{\alpha}|x_t^{\alpha})Q^{\alpha}(x_{t+1}^{\alpha}|x_t^{\alpha},a_t^{\alpha},\mu^G_t;g^{\alpha})$. We note that the solution of~\eqref{eq:m_FP}, $\tgamma_t$, appears both on the left of~\eqref{eq:m_FP} and on the right side in the update of $\mu^G_t$, and is thus unlike the fixed-point equation found in Bayesian Nash equilibrium.

			Furthermore, using the quantity $\tilde{\gamma}_t$ found above, define
			\begin{align}
				V^{\alpha}_{t}(\mu^G_t,x_t^{\alpha})\defeq\E^{\tilde{\gamma}_t(\cdot|x^{\alpha})}\left[R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha})+\delta V^{\alpha}_{t+1}(\phi(\mu^G_t,\tgamma_t), X_{t+1}^{\alpha}) | \mu^G_t,x_t^{\alpha}\right].  \label{eq:Vdef}
			\end{align}
   		\end{enumerate}
		Then, an equilibrium strategy is defined as 
		\begin{align}
			\tilde{\sigma}_t^{\alpha}(a_t^{\alpha}|\mu^G_{1:t},x_{1:t}^{\alpha}) = \tilde{\gamma}_t(a_t^{\alpha}|x_t^{\alpha}), \label{eq:sigma_fh}
		\end{align}
		where $\tilde{\gamma}_t = \theta[\mu^G_t]$. 

		In the following theorem, we show that the strategy thus constructed is a \glspl{gmfg} of the game.

%%%%%%%%%%%%%
		\begin{theorem}
		\label{Thm:Main}
			A strategy $(\tsigma)$ constructed from the above algorithm is an \mpe of the game i.e. $\forall t, h^{\alpha}_t \in \cH^{\alpha}_t, {\sigma^{\alpha}}$,
			\begin{align}
				\label{eq:prop}
				\E^{(\tsigma^{\alpha} \tsigma^{-\alpha})}&\left[\sum_{n=t}^T \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] \geq \nn\\
				&\E^{({\sigma}^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^T \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] 
			\end{align}
		\end{theorem}
		\begin{proof}
			Please see Appendix~\ref{app:A}.
		\end{proof}

	\subsection{Converse}
		In the following, we show that every \gmfe can be found using the above backward recursion.

		\begin{theorem}[Converse]
		\label{thm:2}
			Let $\tsigma$ be a \gmfe of the graphon mean field game. Then there exists an equilibrium generating function $\theta$ that satisfies \eqref{eq:m_FP} in backward recursion such that  $\tsigma$ is defined using $\theta$.
		\end{theorem}
		\begin{proof}
			Please see Appendix~\ref{app:C}.
		\end{proof}

	\subsection{Backward recursive algorithm for $\mathbb{G}_{\infty}$} \label{sec:fhbr}
		In this section, we consider the infinite-horizon problem $\mathbb{G}_{\infty}$, for which we assume the reward function $R$ to be absolutely bounded.

		We define an equilibrium generating function $\theta:\cZ\to\{\cX\to\mathcal{P}(\cA) \}$, where for each $\mu^G_t $, we generate $\tgamma_t = \theta[\mu^G_t]$. In addition, we generate a reward-to-go function $V:\cZ\times\cX\to\mathbb{R}$.
		These quantities are generated through a fixed-point equation as follows.

		For all $\mu^G,$ set $\tilde{\gamma} = \theta[z]$. Then $(\tilde{\gamma},V)$ are solution of the following fixed-point equation\footnote{We discuss the existence of solution of this fixed-point equation in Section~\ref{sec:exists}}, $\forall z\in\cZ,x^{\alpha}\in \cX$,
		\begin{align}
			\label{eq:m_FP_ih}
			\tilde{\gamma}(\cdot|x^{\alpha}) \in \arg\max_{\gamma(\cdot|x^{\alpha})}&\E^{\gamma(\cdot|x^{\alpha})} \left[R(x^{\alpha},A^{\alpha},\mu^G;g^{\alpha})+\delta V(\phi(\mu^G,\tgamma), X^{{\alpha}'};g^{\alpha}) | \mu^G,x^{\alpha}\right] ,\\
			V(z,x^{\alpha}) =\  &\E^{\tilde{\gamma}(\cdot|x^{\alpha})} \left[ R(x^{\alpha},A^{\alpha},\mu^G;g^{\alpha})+\delta V (\phi(\mu^G,\tgamma;g^{\alpha}), X^{{\alpha}'}) | \mu^G,x^{\alpha}\right]. 
		\end{align}
 		where expectation in \eqref{eq:m_FP_ih} is with respect to random variable $(A^{\alpha},X^{{\alpha},\prime})$ through the measure $\gamma(a^{\alpha}|x^{\alpha})Q^{\alpha}(x^{{\alpha}'}|x^{\alpha},a^{\alpha},\mu^G)$.

		Then an equilibrium strategy is defined as 
		\begin{align}
			\tilde{\sigma}^{\alpha}(a_t^{\alpha}|\mu^G_{1:t},x_{1:t}^{\alpha}) = \tilde{\gamma}(a_t^{\alpha}|x_t^{\alpha}), \label{eq:sigma_ih}
		\end{align}
		where $\tilde{\gamma} = \theta[\mu^G_t]$.

		The following theorem shows that the strategy thus constructed is a \gmfe of the game.

		\begin{theorem}
		\label{thih}
			A strategy $(\tsigma)$ constructed from the above algorithm is a \gmfe of the game i.e. $\forall t, h^{\alpha}_t \in \cH^{\alpha}_t, {\sigma^{\alpha}}$,

			\begin{align}
				\label{eq:prop_ih}
				\E^{(\tsigma^{\alpha} \tsigma^{-\alpha})}&\left[\sum_{n=t}^\infty \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] \geq\nn\\
				&\E^{({\sigma}^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^\infty \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right], 
			\end{align} 
		\end{theorem}
		\begin{proof}
			Please see Appendix~\ref{app:D}.
		\end{proof}

	\subsection{Converse}
		In the following, we show that every \gmfe can be found using the above backward recursion.
		\begin{theorem}[Converse]
		\label{thm:2ih}
			Let $\tsigma$ be a \gmfe the graphon mean field game. Then there exists an equilibrium generating function $\theta$
			that satisfies \eqref{eq:m_FP} in backward recursion such that  $\tsigma$ is defined using $\theta$.
		\end{theorem}
		\begin{proof}
			Please see Appendix~\ref{app:idih}.
		\end{proof}




==> 4Method.tex <==
	\label{sec:methodology}
	In this section, we will provide a backward recursive methodology to compute \glspl{gmfg} for both $\mathbb{G}_{T}$ and $\mathbb{G}_{\infty}$. We will consider Markovian equilibrium strategies of player $\alpha$ which depend on the common information at time $t$, $\mu^G_{t}$, and on its current type $x_t^{\alpha}$.\footnote{Note however, that the unilateral deviations of the player are considered in the space of all strategies.}  Equivalently, player $\alpha$ takes action of the form $A_t^{\alpha}\sim \sigma_t^{\alpha}(\cdot|\mu^G_t,x_t^{\alpha})$. Similar to the common agent approach in~\cite{NaMaTe13}, an alternate and equivalent way of defining the strategies of the players is as follows. We first generate partial function $\gamma_t^{\alpha}:\cX\to\cP(\cA)$ as a function of $\mu^G_t$ through an equilibrium generating function $\theta_t^{\alpha}:\cZ\to(\cX\to\cP(\cA))$ such that $\gamma_t^{\alpha} = \theta_t^{\alpha}[\mu^G_t]$. Then action $A_t^{\alpha}$ is generated by applying this prescription function $\gamma_t^{\alpha}$ on player $\alpha$'s current private information $x_t^{\alpha}$, i.e. $A_t^{\alpha}\sim \gamma_t^{\alpha}(\cdot|x_t^{\alpha})$. Thus $A_t^{\alpha}\sim \sigma_t^{\alpha}(\cdot|\mu^G_{t},x_t^{\alpha}) = \theta_t^{\alpha}[\mu^G_t](\cdot|x_t^{\alpha})$.
	
	For a given prescription function $\gamma^{\alpha}_t = \theta^{\alpha}[\mu^G_t]$, the graphon mean-field $\mu^G_t$ evolves according to the discrete-time McKean Vlasov equation, $\forall y\in\cX$ and $\forall \alpha\in[0,1]$:
	\begin{align}
		\mu^{\alpha}_{t+1}(y) =\sum_{x\in\cX}\sum_{a\in \cA} \mu^{\alpha}_t(x)\gamma^{\alpha}_t(a|x)Q\left(y|x,a,\mu^G_t;g^{\alpha}\right), \label{eq:muG_update}
	\end{align}
	which implies
	\begin{align}
		\mu^{\alpha}_{t+1}&= \phi^{\alpha}(\mu^{\alpha}_t,\gamma^{\alpha}_t,\mu^G_t;g^{\alpha})\\
		\mu_{t+1}^G &= \phi(\mu_t^G,\gamma_t;g^{\alpha}) 
	\end{align}

	\subsection{Backward recursive algorithm for $\mathbb{G}_{T}$} \label{sec:fhbr1}
		In this subsection, we will provide a methodology to generate \gmfe of $\mathbb{G}_{T}$ of the form described above. We define an equilibrium generating function $(\theta_t)_{t\in[T]}$, where $\theta_t:\cZ\to\{\cX\to\mathcal{P}(\cA) \}$, where for each $\mu^G_t $, we generate $\tgamma_t = \theta_t[\mu^G_t]$. In addition, we generate a reward-to-go function $(V^{\alpha}_t)_{t\in[T]}$, where $V^{\alpha}_t:\cZ\times\cX\to\mathbb{R}$. These quantities are generated through a fixed-point equation as follows.
		\begin{enumerate}
			\item Initialize $\forall \mu^G_{T+1}, x_{T+1}^{\alpha}\in \cX$,
			\begin{align}
				V^{\alpha}_{T+1}(\mu^G_{T+1},x_{T+1}^{\alpha}) \defeq 0.   \label{eq:VT+1}
			\end{align}

			\item For $t = T,T-1, \ldots 1, \ \forall \mu^G_t$, let $\theta_t[\mu^G_t] $ be generated as follows. Set $\tilde{\gamma}_t = \theta_t[\mu^G_t]$, where $\tilde{\gamma}_t$ is the solution of the following fixed-point equation\footnote{We discuss the existence of solution of this fixed-point equation in Section~\ref{sec:exists}}, $\forall i \in [N],x_t^{\alpha}\in \cX$,
  			\begin{align}
				 \tilde{\gamma}_t(\cdot|x_t^{\alpha}) \in  \arg\max_{\gamma_t(\cdot|x_t^{\alpha})} \E^{\gamma_t(\cdot|x_t^{\alpha})}\left[ R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha})+\delta V^{\alpha}_{t+1}(\phi(\mu^G_t,\tgamma_t;g^{\alpha}), X_{t+1}^{\alpha}) | \mu^G_t,x_t^{\alpha}\right] , \label{eq:m_FP}
			\end{align}
 			where expectation in \eqref{eq:m_FP} is with respect to random variable $(A_t^{\alpha},X_{t+1}^{\alpha})$ through the probability measure $\gamma_t(a_t^{\alpha}|x_t^{\alpha})Q^{\alpha}(x_{t+1}^{\alpha}|x_t^{\alpha},a_t^{\alpha},\mu^G_t;g^{\alpha})$. We note that the solution of~\eqref{eq:m_FP}, $\tgamma_t$, appears both on the left of~\eqref{eq:m_FP} and on the right side in the update of $\mu^G_t$, and is thus unlike the fixed-point equation found in Bayesian Nash equilibrium.

			Furthermore, using the quantity $\tilde{\gamma}_t$ found above, define
			\begin{align}
				V^{\alpha}_{t}(\mu^G_t,x_t^{\alpha})\defeq\E^{\tilde{\gamma}_t(\cdot|x^{\alpha})}\left[R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha})+\delta V^{\alpha}_{t+1}(\phi(\mu^G_t,\tgamma_t), X_{t+1}^{\alpha}) | \mu^G_t,x_t^{\alpha}\right].  \label{eq:Vdef}
			\end{align}
   		\end{enumerate}
		Then, an equilibrium strategy is defined as 
		\begin{align}
			\tilde{\sigma}_t^{\alpha}(a_t^{\alpha}|\mu^G_{1:t},x_{1:t}^{\alpha}) = \tilde{\gamma}_t(a_t^{\alpha}|x_t^{\alpha}), \label{eq:sigma_fh}
		\end{align}
		where $\tilde{\gamma}_t = \theta[\mu^G_t]$. 

		In the following theorem, we show that the strategy thus constructed is a \glspl{gmfg} of the game.

%%%%%%%%%%%%%
		\begin{theorem}
		\label{Thm:Main}
			A strategy $(\tsigma)$ constructed from the above algorithm is an \mpe of the game i.e. $\forall t, h^{\alpha}_t \in \cH^{\alpha}_t, {\sigma^{\alpha}}$,
			\begin{align}
				\label{eq:prop}
				\E^{(\tsigma^{\alpha} \tsigma^{-\alpha})}&\left[\sum_{n=t}^T \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] \geq \nn\\
				&\E^{({\sigma}^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^T \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] 
			\end{align}
		\end{theorem}
		\begin{proof}
			Please see Appendix~\ref{app:A}.
		\end{proof}

	\subsection{Converse}
		In the following, we show that every \gmfe can be found using the above backward recursion.

		\begin{theorem}[Converse]
		\label{thm:2}
			Let $\tsigma$ be a \gmfe of the graphon mean field game. Then there exists an equilibrium generating function $\theta$ that satisfies \eqref{eq:m_FP} in backward recursion such that  $\tsigma$ is defined using $\theta$.
		\end{theorem}
		\begin{proof}
			Please see Appendix~\ref{app:C}.
		\end{proof}

	\subsection{Backward recursive algorithm for $\mathbb{G}_{\infty}$} \label{sec:fhbr}
		In this section, we consider the infinite-horizon problem $\mathbb{G}_{\infty}$, for which we assume the reward function $R$ to be absolutely bounded.

		We define an equilibrium generating function $\theta:\cZ\to\{\cX\to\mathcal{P}(\cA) \}$, where for each $\mu^G_t $, we generate $\tgamma_t = \theta[\mu^G_t]$. In addition, we generate a reward-to-go function $V:\cZ\times\cX\to\mathbb{R}$.
		These quantities are generated through a fixed-point equation as follows.

		For all $\mu^G,$ set $\tilde{\gamma} = \theta[z]$. Then $(\tilde{\gamma},V)$ are solution of the following fixed-point equation\footnote{We discuss the existence of solution of this fixed-point equation in Section~\ref{sec:exists}}, $\forall z\in\cZ,x^{\alpha}\in \cX$,
		\begin{align}
			\label{eq:m_FP_ih}
			\tilde{\gamma}(\cdot|x^{\alpha}) \in \arg\max_{\gamma(\cdot|x^{\alpha})}&\E^{\gamma(\cdot|x^{\alpha})} \left[R(x^{\alpha},A^{\alpha},\mu^G;g^{\alpha})+\delta V(\phi(\mu^G,\tgamma), X^{{\alpha}'};g^{\alpha}) | \mu^G,x^{\alpha}\right] ,\\
			V(z,x^{\alpha}) =\  &\E^{\tilde{\gamma}(\cdot|x^{\alpha})} \left[ R(x^{\alpha},A^{\alpha},\mu^G;g^{\alpha})+\delta V (\phi(\mu^G,\tgamma;g^{\alpha}), X^{{\alpha}'}) | \mu^G,x^{\alpha}\right]. 
		\end{align}
 		where expectation in \eqref{eq:m_FP_ih} is with respect to random variable $(A^{\alpha},X^{{\alpha},\prime})$ through the measure $\gamma(a^{\alpha}|x^{\alpha})Q^{\alpha}(x^{{\alpha}'}|x^{\alpha},a^{\alpha},\mu^G)$.

		Then an equilibrium strategy is defined as 
		\begin{align}
			\tilde{\sigma}^{\alpha}(a_t^{\alpha}|\mu^G_{1:t},x_{1:t}^{\alpha}) = \tilde{\gamma}(a_t^{\alpha}|x_t^{\alpha}), \label{eq:sigma_ih}
		\end{align}
		where $\tilde{\gamma} = \theta[\mu^G_t]$.

		The following theorem shows that the strategy thus constructed is a \gmfe of the game.

		\begin{theorem}
		\label{thih}
			A strategy $(\tsigma)$ constructed from the above algorithm is a \gmfe of the game i.e. $\forall t, h^{\alpha}_t \in \cH^{\alpha}_t, {\sigma^{\alpha}}$,

			\begin{align}
				\label{eq:prop_ih}
				\E^{(\tsigma^{\alpha} \tsigma^{-\alpha})}&\left[\sum_{n=t}^\infty \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] \geq\nn\\
				&\E^{({\sigma}^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^\infty \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right], 
			\end{align} 
		\end{theorem}
		\begin{proof}
			Please see Appendix~\ref{app:D}.
		\end{proof}

	\subsection{Converse}
		In the following, we show that every \gmfe can be found using the above backward recursion.
		\begin{theorem}[Converse]
		\label{thm:2ih}
			Let $\tsigma$ be a \gmfe the graphon mean field game. Then there exists an equilibrium generating function $\theta$
			that satisfies \eqref{eq:m_FP} in backward recursion such that  $\tsigma$ is defined using $\theta$.
		\end{theorem}
		\begin{proof}
			Please see Appendix~\ref{app:idih}.
		\end{proof}




==> Arxiv/0config.tex <==
\usepackage{bbm}
\usepackage{amsmath}
\usepackage{mathrsfs}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{amsfonts}
\usepackage[english]{babel}
\usepackage{amsthm}
\usepackage{epstopdf}


\newtheorem{theorem}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{fact}{Fact}
\newtheorem{problem}{Problem}
\newtheorem{lemma*}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}



\newcommand{\mA}{\mathcal{A}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mN}{[N]}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cV}{\mathcal{V}}

\renewcommand{\hat}{\widehat}
\renewcommand{\bar}{\overline}
\newcommand{\ux}{\underline{x}}
\renewcommand{\star}{\ast}
\def\lpr{\left\{}
\def\rpr{\right\}}
\newcommand{\uF}{F}
\newcommand{\mP}{\mathbb{P}}
\newcommand{\mE}{\mathbb{E}}	
\newcommand\addtag{\refstepcounter{equation}\tag{\theequation}}
\newcommand{\eq}[1]{\begin{align}#1\end{align}}
\newcommand{\seq}[1]{\begin{subequations}#1\end{subequations}}

\newcommand{\lb}[1]{\left\{ \begin{array}{ll} #1 \end{array} \right.}
\newcommand*\dif{\mathop{}\!\mathrm{d}}
\newcommand{\bm}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\E}{\mathbb{E}}
 \newcommand{\nn}{\nonumber}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cZ}{\mu^G}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\tsigma}{\tilde{\sigma}}
\newcommand{\hmu}{\hat{\mu}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\tgamma}{\tilde{\gamma}}
\newcommand{\Qx}[1]{Q^{\alpha}(#1)}
\newcommand{\Qv}[1]{Q_v^{\alpha}(#1)}
\newcommand{\defeq}{\buildrel\triangle\over =}
\newcommand{\apos}{\textsc{\char13}}
\newcommand{\tred}[1]{\textcolor{red}{#1}}
\newcommand{\pushright}[1]{\ifmeasuring@ #1 \else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@ #1 \else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\newcommand{\hs}[1]{\hspace{#1}}


==> Arxiv/0glossary.tex <==
\usepackage{xspace}
\usepackage[acronym,nogroupskip,nonumberlist,nopostdot]{glossaries}
\glsdisablehyper

% WIRELESS AND DIGITAL COMMS
\newacronym{mdp}{MDP}{Markov decision process}
\newacronym{ne}{NE}{Nash equillibrium}
\newacronym{mfe}{MFE}{mean-field equillibrium}
\newacronym{mpe}{MPE}{Markov perfect equillibrium}
\newacronym{mfg}{MFG}{mean-field game}
\newacronym{rl}{RL}{reinforcement learning}
\newacronym{marl}{MARL}{multi-agent reinforcement learning}
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{ssg}{SSG}{Stackelberg security game}
\newacronym{pse}{PSE}{perfect Stackelberg equilibrium}
\newacronym{mpse}{MPSE}{Markov \gls{pse}}
\newacronym{pomdp}{POMDP}{partially observed \gls{mdp}}
\newacronym{mc}{MC}{Monte Carlo}
\newacronym{pbe}{PBE}{perfect Bayesian equilibrium}
\newacronym{gmfg}{GMFG}{graphon mean-field game}
\newacronym{gmfe}{GMFE}{graphon mean-field equillibrium}
\newacronym{spe}{SPE}{sub-game perfect equillibrium}
\newacronym{mkv}{MKV}{McKean-Vlasov}

\newcommand{\mdp}{\gls{mdp}\xspace}
\newcommand{\gne}{\gls{ne}\xspace}
\newcommand{\mfe}{\gls{mfe}\xspace}
\newcommand{\mpe}{\gls{mpe}\xspace}
\newcommand{\mfg}{\gls{mfg}\xspace}
\newcommand{\mfgs}{\glspl{mfg}\xspace}
\newcommand{\rl}{\gls{rl}\xspace}
\newcommand{\marl}{\gls{marl}\xspace}
\newcommand{\ssg}{\gls{ssg}\xspace}
\newcommand{\ssgs}{\glspl{ssg}\xspace}
\newcommand{\pse}{\gls{pse}\xspace}
\newcommand{\mpse}{\gls{mpse}\xspace}
\newcommand{\pomdp}{\gls{pomdp}\xspace}
\newcommand{\pbe}{\gls{pbe}\xspace}
\newcommand{\gmfg}{\gls{gmfg}\xspace}
\newcommand{\gmfe}{\gls{gmfe}\xspace}
\newcommand{\spe}{\gls{spe}\xspace}
\newcommand{\spes}{\glspl{spe}\xspace}
\newcommand{\mkv}{\gls{mkv}\xspace}

==> Arxiv/1Introduction.tex <==
Strategic interaction of interconnected agents has been an important topic of study for many decades and its relevance has been increasing rapidly with the progress of internet penetration and smartphone devices in our society. The recent decade has seen tremendous technological advancement in the field of networking applications that has led to an unprecedented scale of interaction among people and devices such as in ride sharing platforms, social media apps, cyber-physical systems, large scale renewable energy, electric vehicles, cryptocurrencies and smart grid systems. For instance, the influence of social networks in the decision making of majority of individuals is a known phenomenon. Most decisions by individuals from which products to buy to whom to vote for are influenced by friends and acquaintances. The emerging empirical evidence on these issues motivates the theoretical study of network effects with strategic agents. The analysis, design and control of such systems that involve strategic interactions embedded in a networked environment could lead to more intelligent and efficient applications, and can enhance our understanding of the mechanics of such interactions. 

Many of the above mentioned applications of interest have following key features: (a) large number of strategic players (b) dynamically evolving incomplete information, and (c) an underlying network. Game theory is a natural choice to model such interactions where the payoffs obtained by individuals depend on the action of her neighbors. A shortcoming of the standard approach to solve dynamic network games with incomplete information is interdependence of strategies of the players across time. Moreover, as the number of players become large as is the case in many practical scenarios considered here, computing Nash equilibrium becomes intractable. 

\subsection{Relevant Literature}
Maskin and Tirole in~\cite{MaTi01} introduced the concept of \mpe for dynamic games governed by an underlying \mdp. The strategies thus computed depend on the present state and not on the past trajectory of the game. In general, there exists a backward recursive methodology to compute \mpe of the game. Some prominent examples of the application of \mpe include~\cite{ErPa95, BeVa96, AcRo01}. Ericson and Pakes in~\cite{ErPa95} model industry dynamics for firms' entry, exit and investment participation, through a dynamic game with symmetric information, compute its \mpe, and prove ergodicity of the equilibrium process. Bergemann and V{\" a}lim{\"a}ki in~\cite{BeVa96} study a learning process in a dynamic oligopoly with strategic sellers and a single buyer, allowing for price competition among sellers. They study \mpe of the game and its convergence behavior. Acemo\u{g}lu and Robinson in~\cite{AcRo01} develop a theory of political transitions in a country by modeling it as a repeated game between the elites and the poor, and study its \mpe.

In large population games, computing \mpe with the methods specified above becomes intractable. Mean field games (MFG) were introduced in Huang, Malham\'e,and Caines~\cite{HuMaCa06}, and Lasry and Lions~\cite{LaLi07} to model the strategic interactions with large number of players. In such games, the individual agents have minimal impact of the overall outcome of the game and so the agents track a mean distribution of states of other agents rather than their actual states. MFGs is an excellent and a tractable model to study large population dynamic games of incomplete information, and has been shown to be a good approximation of Nash equilibrium (or MPE) of the original game as the number of players grow large (for instance see ~\cite{Caetal15,La16,Fi17,La18,DeLaRa19} and references therein).

Parise and Ozdaglar introduced the notion of graphon games~\cite{PaOz19} to model large population \emph{static} network games, where graphon is generative model of a large random graph inroduced by Lov\"asz in~\cite{Lo12}. Caines and Huang in~\cite{CaHu18} combined the ideas of \mfe and graphon games to define Graphon Mean field games (\glspl{gmfg}) where there are a large number of strategic agents with dynamic incomplete information who interact on an underlying fixed network generated by a known graphon. 
\glspl{gmfg} combine the idea of network games defined through graphons and the mean field framework of describing multi agent homogeneous games and predicting equilibrium in a tractable manner. Large network of nodes interacting with one another can be represented as graphons and mean field games deal with the study of such large interaction among devices and people as agents to analyze such systems to design and understand the behavior of such large scale interactions and their impact on our society. The progress in research in the mean field domain have been restricted to cases where the agents interacted in a perfect homogeneous environment and the interactions between the agents were assumed to be uniform irrespective of the location of the agent in the network. What if, the population interaction was not uniform and there was a measure of how the agents interacted with each other or in other words, the payoff and the transition to the next state was conditional on the relative position of the agent in the network. The mean field distribution would be affected by it so will the optimum policies and the Nash equilibrium thus generated. The theoretical basis for such a case has been provided in~\cite{CaHu18} which generalizes the idea of mean field games across the population with different levels of interactions through \gmfg. In this paper, we propose a sequential decomposition algorithm to compute \glspl{gmfg} by decomposing the problem across time, which reduces the complexity of computing \glspl{gmfg} from exponential to linear in time. 
 
We consider a discounted infinite-horizon dynamic graphon mean-field game where there is a large population of homogeneous players each having a private type. Each player sequentially makes strategic decisions and is affected by other players in its neighborhood through a graphon mean-field population state. Each player has a private type that evolves through a controlled Markov process as a function of the graphon, which only she observes and all players observe a common population state which is the distribution of other players' types. In such games, the graphon mean-field state evolves through McKean-Vlasov forward equation given a policy of the players and the graphon function. The equilibrium policy satisfies the Bellman backward equation, given the graphon mean-field states. Thus to compute equilibrium, one needs to solve the coupled backward and forward fixed-point equation in the graphon mean-field and the equilibrium policy. 

In order to demonstrate the utility of our algorithm to compute the \gmfe of a graphon mean field game for varying graphons, we consider a cyber-security example of malware spread problem.  A cluster of nodes in a network of physical servers get infected by an independent random process. For each node, there is a higher risk of getting infected due to negative externality imposed by other infected players. A graphon function is defined that quantifies the effect of the effect of the state of other nodes in the network on the concerned node. At each time t, a node privately observes its own state and publicly observes the population of infected nodes, based on which it has to make a decision to repair or not. Upon taking an action, the transition of to the  next state is governed by both its individual action and the actions affected by the neighboring agents given by a graphon function. Using our algorithm, we find equilibrium strategies of the players which are observed to be non-decreasing in the healthy population state. 

The paper is structured as follows. In Section~\ref{sec:Model}, we present a model of the graphon mean field game, followed by some preliminary result from our past research regarding \mpe in strategic dynamic games. In section ~\ref{sec:methodology}, we present our main results where we present algorithm to compute \mpe for both finite and infinite horizon game, and also present existence results. In section ~\ref{sec:example}, we show the simulation results for the cyber-security example assuming different graphons and conclude in Section~\ref{sec:Concl}.

\subsection{Notation}
	We use uppercase letters for random variables and lowercase for their realizations. For any variable, subscripts represent time indices and superscripts represent player identities. We use notation $ -\alpha$ to represent all players other than player $\alpha$ i.e. $ -\alpha = \{1,2, \ldots i-1, i+1, \ldots, N \}$. We use notation $a_{t:t'}$ to represent the vector $(a_t, a_{t+1}, \ldots a_{t'})$ when $t'\geq t$ or an empty vector if $t'< t$. We use $a_t^{-\alpha}$ to mean $(a^1_t, a^2_{t}, \ldots, a_t^{i-1}, a_t^{i+1} \ldots, a^N_{t})$. We use the notation $\sum_x$ to represent both $\sum_x$ and $\int_x$, and the correct usage is determined depending on the space of $x$. We remove superscripts or subscripts if we want to represent the 
	 vector, for example $a_t$  represents $(a_t^1, \ldots, a_t^N) $. We denote the indicator function of any set $A$ by $\mathbbm{1}\{A\}$. For any finite set $\mathcal{S}$, $\mathcal{P}(\mathcal{S})$ represents space of probability measures on $\mathcal{S}$ and $|\mathcal{S}|$ represents its cardinality. We denote by $P^{\sigma}$ (or $E^{\sigma}$) the probability measure generated by (or expectation with respect to) strategy profile $\sigma$. We denote the set of real numbers by $\mathbb{R}$. For a probabilistic strategy profile of players $(\sigma_t^{\alpha})_{i\in [N]}$ where probability of action $a_t^{\alpha}$ conditioned on $\mu^G_{1:t},x_{1:t}^{\alpha}$ is given by $\sigma_t^{\alpha}(a_t^{\alpha}|\mu^G_{1:t},x_{1:t}^{\alpha})$, we use the short hand notation $\sigma_t^{-\alpha}(a_t^{-\alpha}|\mu^G_{1:t},x_{1:t}^{-\alpha})$ to represent $\prod_{j\neq i} \sigma_t^j(a_t^j|\mu^G_{1:t},x_{1:t}^j)$. All equalities and inequalities involving random variables are to be interpreted in \emph{a.s.} sense.


==> Arxiv/2Model.tex <==
	\label{sec:Model}
	\subsection{Graphon Mean Field Games}
		Let us consider a discrete-time large population sequential game with $N$ homogeneous players with $N\to\infty$. The interactions between these $N$ players are captured in a asymptotically infinite network graph represented as a \emph{graphon}. Graphons are bounded symmetric Lebesgue measurable functions $W:\left[0,1\right]^2\to\left[0,1\right]$ which can be represented as weighted graphs on the vertex set $\left[0,1\right]$ such that $\mathbf{G}=\left\{g\left(\alpha,\beta\right):0\leq\alpha,\beta\leq 1\right\}$~\cite{CaHu18}. It is similar to an adjacency matrix defined over a $2$-dimensional plane where each entry in the matrix is the measure of coupling between the agents concerned. 
				
		In each period $t\in[T]$, where $[T]$ represents the time horizon, a player $\alpha\in\left[0,1\right]$ observes a private type $x_t^{\alpha}\in\cX$ and a common observation $\mu_t^G$, then takes an action $a_t^{\alpha}\in\cA $ and receives a reward $R(x_t^{\alpha},a_t^{\alpha},\mu_t^G)$. The common observation is an ensemble of the mean field distributions with respect to all agents $\alpha\in[0,1]$ given as $\mu^G_t = \{\mu_t^{\alpha}\}_{{\alpha}}$ where 	
		\begin{align}
			\mu_t^\alpha\left(x\right)=\mathbbm{P}\left\{x_t^\alpha=x\right\}
		\end{align}	
		with $\sum_{i=1}^{N_x} \mu^{\alpha}_t(i) = 1$. Player $\alpha$'s type evolves as a controlled Markov process,	
		\begin{align}
			\label{eqn:markov}
			x_{t+1}^{\alpha} = \tilde{f}[x_t^{\alpha} , a_t^{\alpha},  \mu_t^G; g^{\alpha} ] + w_t^{\alpha}.
		\end{align}

		The random variables $(w_t^{\alpha})_{{\alpha},t}$ are assumed to be mutually independent across players and across time. We also write the above update of $x_t^{\alpha}$ through a kernel, $x_{t+1}^{\alpha}\sim Q^{\alpha}(\cdot|x_t^{\alpha}, a_t^{\alpha}, \mu^G_t;g^{\alpha})$ which depends on the graphon function $g^\alpha=\left\{g(\alpha,\beta):0\leq\beta\leq1\right\}$. 
		
		The dynamics of the \mdp are governed both by the local information as well as the global dynamics involving the effect of the policy action of other players in the system. The idea of graphon is to capture the effect of the actions of all the other players $\beta\in[0,1]$ on player $\alpha$. In prior mean field research, it was assumed that there is a perfect interaction between the players and also that these interactions were uniform. In~\cite{CaHu18}, they provide a set of differential equations that govern such interactions in the mean field setting. The functions below show how the graphon is used in determining the effect of players on one another. The function $\tilde{f}$ in~\eqref{eqn:markov} is given as		
		\begin{align}
			\label{eq:func1}
			\tilde{f}[x_t^{\alpha} , a_t^{\alpha},  \mu_t^G; g^{\alpha} ] = f_0\left(x_t^{\alpha} , a_t^{\alpha}\right) + f\left[x_t^{\alpha} , a_t^{\alpha},  \mu_t^G; g^{\alpha} \right]
		\end{align}
		where
		\begin{align}
			\label{eq:func2}
			f\left[x_t^{\alpha} , a_t^{\alpha},  \mu_t^G; g^{\alpha} \right] =	\int_{\beta\in[0,1]}\sum_{x^\beta\in\cX}&f\left(x^\alpha_t,a^\alpha_t,x^\beta\right)g\left(\alpha,\beta\right)\mu_t^\beta(x^\beta)d(x^\beta)d\beta 		
		\end{align}
		and $f_0$ represent the local effect of the agent when it takes any action and is independent of the actions taken by other agents. In the case, when the agents do not interact at all i.e. $g(\alpha,\beta)=0$, the markov process reduces only to the function $f_0$ ignoring the degenerate case when $\alpha=\beta$. 
		
		At instant $t$, the player $\alpha$ observes the trajectory $(\mu^G_{1:t},x_{1:t}^{\alpha})$ and takes an action $a_t^{\alpha}$ according to a behavioral strategy $\sigma^{\alpha} = (\sigma_t^{\alpha})^t$, where $\sigma_t^{\alpha}:(\mu^G)^{t}\times\mathcal{X}^t \to \mathcal{P}(\mathcal{A})$. We denote the space of such strategies as $\mathcal{K}^{\sigma}$. This implies $A_t^{\alpha}\sim \sigma_t^{\alpha}(\cdot|\mu^G_{1:t},x_{1:t}^{\alpha})$. We denote $\mathcal{Z}^t$ to be the space of population states $\mu^G_{1:t}$ till time $t$. We denote $\mathcal{H}_t^{\alpha}=\mathcal{Z}^t \times \mathcal{X}^t$ to be set of observed histories $(\mu^G_{1:t},x_{1:t}^{\alpha})$ of player $\alpha$.

		For finite time-horizon game, $\mathbb{G}_{T}$, each player wants to maximize its total expected discounted reward over a time horizon $T$, discounted by discount factor $0<\delta\leq1$, 
		\begin{align}
			J^{\alpha,T} :=\E^{\sigma} \left[\sum_{t=1}^T \delta^{t-1} R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha}) \right].
		\end{align} 

		For the infinite time-horizon game, $\mathbb{G}_{\infty}$, each player wants to maximize its total expected discounted reward over an infinite-time horizon discounted by a discount factor $0<\delta<1$, 
		\begin{align}
			J^{\alpha,\infty} :=\E^{\sigma} \left[\sum_{t=1}^\infty \delta^{t-1} R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha}) \right].
		\end{align} 

	\subsection{Solution concept: \mpe}
		The Nash equilibrium (NE) of $\mathbb{G}_{T}$ is defined as strategies $\tsigma = (\tsigma_t^{\alpha})_{\alpha\in\left[0,1\right],t\in\left[T\right]}$ that satisfy, for all $\alpha\in\left[0,1\right]$, 
		\begin{align}
			\E^{(\tsigma^{\alpha},\tsigma^{-\alpha})}\left[\sum_{t=1}^T \delta^{t-1} R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha}) \right]\geq \E^{(\sigma^{\alpha},\tsigma^{-\alpha})}\left[\sum_{t=1}^T \delta^{t-1} R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha})\right],
		\end{align} 
		For sequential games, however, a more appropriate equilibrium concept is \mpe~\cite{MaTi01}, which we use in this paper. We note that an \mpe is also a Nash equilibrium of the game, although not every Nash equilibrium is an \mpe. An \mpe $(\tsigma)$ satisfies sequential rationality such that for $\mathbb{G}_T$, $\forall\alpha\in\left[0,1\right], t \in \left[T\right], h^{\alpha}_t \in \cH^{\alpha}_t, {\sigma^{\alpha}}$,
		\begin{align}
			\E^{(\tsigma^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^T\delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] \geq
			\E^{({\sigma}^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^T \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right], \;\; \;\;   \label{eq:seqeq2}
		\end{align}
		NE and \mpe for $\mathbb{G}_{\infty}$ are defined in a similar way where summation in the above equations is taken such that $T$ is replaced by $\infty$.

==> Arxiv/3Method.tex <==
	\label{sec:methodology}
	In this section, we will provide a backward recursive methodology to compute \glspl{gmfg} for both $\mathbb{G}_{T}$ and $\mathbb{G}_{\infty}$. We will consider Markovian equilibrium strategies of player $\alpha$ which depend on the common information at time $t$, $\mu^G_{t}$, and on its current type $x_t^{\alpha}$.\footnote{Note however, that the unilateral deviations of the player are considered in the space of all strategies.}  Equivalently, player $\alpha$ takes action of the form $A_t^{\alpha}\sim \sigma_t^{\alpha}(\cdot|\mu^G_t,x_t^{\alpha})$. Similar to the common agent approach in~\cite{NaMaTe13}, an alternate and equivalent way of defining the strategies of the players is as follows. We first generate partial function $\gamma_t^{\alpha}:\cX\to\cP(\cA)$ as a function of $\mu^G_t$ through an equilibrium generating function $\theta_t^{\alpha}:\cZ\to(\cX\to\cP(\cA))$ such that $\gamma_t^{\alpha} = \theta_t^{\alpha}[\mu^G_t]$. Then action $A_t^{\alpha}$ is generated by applying this prescription function $\gamma_t^{\alpha}$ on player $\alpha$'s current private information $x_t^{\alpha}$, i.e. $A_t^{\alpha}\sim \gamma_t^{\alpha}(\cdot|x_t^{\alpha})$. Thus $A_t^{\alpha}\sim \sigma_t^{\alpha}(\cdot|\mu^G_{t},x_t^{\alpha}) = \theta_t^{\alpha}[\mu^G_t](\cdot|x_t^{\alpha})$.
	
	For a given prescription function $\gamma^{\alpha}_t = \theta^{\alpha}[\mu^G_t]$, the graphon mean-field $\mu^G_t$ evolves according to the discrete-time McKean Vlasov equation, $\forall y\in\cX$ and $\forall \alpha\in[0,1]$:
	\begin{align}
		\mu^{\alpha}_{t+1}(y) =\sum_{x\in\cX}\sum_{a\in \cA} \mu^{\alpha}_t(x)\gamma^{\alpha}_t(a|x)Q\left(y|x,a,\mu^G_t;g^{\alpha}\right), \label{eq:muG_update}
	\end{align}
	which implies
	\begin{align}
		\mu^{\alpha}_{t+1}&= \phi(\mu^{\alpha}_t,\gamma^{\alpha}_t,\mu^G_t;g^{\alpha})\\
		\mu_{t+1}^G &= \phi(\mu_t^G,\gamma_t;g^{\alpha}) 
	\end{align}

	\subsection{Backward recursive algorithm for $\mathbb{G}_{T}$} \label{sec:fhbr1}
		In this subsection, we will provide a methodology to generate \gmfe of $\mathbb{G}_{T}$ of the form described above. We define an equilibrium generating function $(\theta_t)_{t\in[T]}$, where $\theta_t:\cZ\to\{\cX\to\mathcal{P}(\cA) \}$, where for each $\mu^G_t $, we generate $\tgamma_t = \theta_t[\mu^G_t]$. In addition, we generate a reward-to-go function $(V^{\alpha}_t)_{t\in[T]}$, where $V^{\alpha}_t:\cZ\times\cX\to\mathbb{R}$. These quantities are generated through a fixed-point equation as follows.
		\begin{enumerate}
			\item Initialize $\forall \mu^G_{T+1}, x_{T+1}^{\alpha}\in \cX$,
			\begin{align}
				V^{\alpha}_{T+1}(\mu^G_{T+1},x_{T+1}^{\alpha}) \defeq 0.   \label{eq:VT+1}
			\end{align}

			\item For $t = T,T-1, \ldots 1, \ \forall \mu^G_t$, let $\theta_t[\mu^G_t] $ be generated as follows. Set $\tilde{\gamma}_t = \theta_t[\mu^G_t]$, where $\tilde{\gamma}_t$ is the solution of the following fixed-point equation\footnote{We discuss the existence of solution of this fixed-point equation in Section~\ref{sec:exists}}, $\forall i \in [N],x_t^{\alpha}\in \cX$,
  			\begin{align}
				 \tilde{\gamma}_t(\cdot|x_t^{\alpha}) \in  \arg\max_{\gamma_t(\cdot|x_t^{\alpha})} \E^{\gamma_t(\cdot|x_t^{\alpha})}\left[ R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha})+\delta V^{\alpha}_{t+1}(\phi(\mu^G_t,\tgamma_t;g^{\alpha}), X_{t+1}^{\alpha}) | \mu^G_t,x_t^{\alpha}\right] , \label{eq:m_FP}
			\end{align}
 			where expectation in \eqref{eq:m_FP} is with respect to random variable $(A_t^{\alpha},X_{t+1}^{\alpha})$ through the probability measure $\gamma_t(a_t^{\alpha}|x_t^{\alpha})Q^{\alpha}(x_{t+1}^{\alpha}|x_t^{\alpha},a_t^{\alpha},\mu^G_t;g^{\alpha})$. We note that the solution of~\eqref{eq:m_FP}, $\tgamma_t$, appears both on the left of~\eqref{eq:m_FP} and on the right side in the update of $\mu^G_t$, and is thus unlike the fixed-point equation found in Bayesian Nash equilibrium.

			Furthermore, using the quantity $\tilde{\gamma}_t$ found above, define
			\begin{align}
				V^{\alpha}_{t}(\mu^G_t,x_t^{\alpha})\defeq\E^{\tilde{\gamma}_t(\cdot|x^{\alpha})}\left[R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha})+\delta V^{\alpha}_{t+1}(\phi(\mu^G_t,\tgamma_t), X_{t+1}^{\alpha}) | \mu^G_t,x_t^{\alpha}\right].  \label{eq:Vdef}
			\end{align}
   		\end{enumerate}
		Then, an equilibrium strategy is defined as 
		\begin{align}
			\tilde{\sigma}_t^{\alpha}(a_t^{\alpha}|\mu^G_{1:t},x_{1:t}^{\alpha}) = \tilde{\gamma}_t(a_t^{\alpha}|x_t^{\alpha}), \label{eq:sigma_fh}
		\end{align}
		where $\tilde{\gamma}_t = \theta[\mu^G_t]$. 

		In the following theorem, we show that the strategy thus constructed is a \glspl{gmfg} of the game.

%%%%%%%%%%%%%
		\begin{theorem}
		\label{Thm:Main}
			A strategy $(\tsigma)$ constructed from the above algorithm is an \mpe of the game i.e. $\forall t, h^{\alpha}_t \in \cH^{\alpha}_t, {\sigma^{\alpha}}$,
			\begin{align}
				\label{eq:prop}
				\E^{(\tsigma^{\alpha} \tsigma^{-\alpha})}&\left[\sum_{n=t}^T \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] \geq \nn\\
				&\E^{({\sigma}^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^T \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] 
			\end{align}
		\end{theorem}
		\begin{proof}
			Please see Appendix~\ref{app:A}.
		\end{proof}

	\subsection{Converse}
		In the following, we show that every \gmfe can be found using the above backward recursion.

		\begin{theorem}[Converse]
		\label{thm:2}
			Let $\tsigma$ be a \gmfe of the graphon mean field game. Then there exists an equilibrium generating function $\theta$ that satisfies \eqref{eq:m_FP} in backward recursion such that  $\tsigma$ is defined using $\theta$.
		\end{theorem}
		\begin{proof}
			Please see Appendix~\ref{app:C}.
		\end{proof}

	\subsection{Backward recursive algorithm for $\mathbb{G}_{\infty}$} \label{sec:fhbr}
		In this section, we consider the infinite-horizon problem $\mathbb{G}_{\infty}$, for which we assume the reward function $R$ to be absolutely bounded.

		We define an equilibrium generating function $\theta:\cZ\to\{\cX\to\mathcal{P}(\cA) \}$, where for each $\mu^G_t $, we generate $\tgamma_t = \theta[\mu^G_t]$. In addition, we generate a reward-to-go function $V:\cZ\times\cX\to\mathbb{R}$.
		These quantities are generated through a fixed-point equation as follows.

		For all $\mu^G,$ set $\tilde{\gamma} = \theta[z]$. Then $(\tilde{\gamma},V)$ are solution of the following fixed-point equation\footnote{We discuss the existence of solution of this fixed-point equation in Section~\ref{sec:exists}}, $\forall z\in\cZ,x^{\alpha}\in \cX$,
		\begin{align}
			\label{eq:m_FP_ih}
			\tilde{\gamma}(\cdot|x^{\alpha}) \in \arg\max_{\gamma(\cdot|x^{\alpha})}&\E^{\gamma(\cdot|x^{\alpha})} \left[R(x^{\alpha},A^{\alpha},\mu^G;g^{\alpha})+\delta V(\phi(z,\tgamma), X^{{\alpha}'};g^{\alpha}) | \mu^G,x^{\alpha}\right] ,\\
			V(z,x^{\alpha}) =\  &\E^{\tilde{\gamma}(\cdot|x^{\alpha})} \left[ R(x^{\alpha},A^{\alpha},\mu^G;g^{\alpha})+\delta V (\phi(\mu^G,\tgamma;g^{\alpha}), X^{{\alpha}'}) | \mu^G,x^{\alpha}\right]. 
		\end{align}
 		where expectation in \eqref{eq:m_FP_ih} is with respect to random variable $(A^{\alpha},X^{{\alpha},\prime})$ through the measure $\gamma(a^{\alpha}|x^{\alpha})Q^{\alpha}(x^{{\alpha}'}|x^{\alpha},a^{\alpha},\mu^G)$.

		Then an equilibrium strategy is defined as 
		\begin{align}
			\tilde{\sigma}^{\alpha}(a_t^{\alpha}|\mu^G_{1:t},x_{1:t}^{\alpha}) = \tilde{\gamma}(a_t^{\alpha}|x_t^{\alpha}), \label{eq:sigma_ih}
		\end{align}
		where $\tilde{\gamma} = \theta[\mu^G_t]$.

		The following theorem shows that the strategy thus constructed is a \gmfe of the game.

		\begin{theorem}
		\label{thih}
			A strategy $(\tsigma)$ constructed from the above algorithm is a \gmfe of the game i.e. $\forall t, h^{\alpha}_t \in \cH^{\alpha}_t, {\sigma^{\alpha}}$,

			\begin{align}
				\label{eq:prop_ih}
				\E^{(\tsigma^{\alpha} \tsigma^{-\alpha})}&\left[\sum_{n=t}^\infty \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] \geq\nn\\
				&\E^{({\sigma}^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^\infty \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right], 
			\end{align} 
		\end{theorem}
		\begin{proof}
			Please see Appendix~\ref{app:D}.
		\end{proof}

	\subsection{Converse}
		In the following, we show that every \gmfe can be found using the above backward recursion.
		\begin{theorem}[Converse]
		\label{thm:2ih}
			Let $\tsigma$ be a \gmfe the graphon mean field game. Then there exists an equilibrium generating function $\theta$
			that satisfies \eqref{eq:m_FP} in backward recursion such that  $\tsigma$ is defined using $\theta$.
		\end{theorem}
		\begin{proof}
			Please see Appendix~\ref{app:idih}.
		\end{proof}




==> Arxiv/4Existence.tex <==
\label{sec:exists}
	In this section, we discuss sufficient conditions for the existence of a solution of the fixed-point equations~\eqref{eq:m_FP} and~\eqref{eq:m_FP_ih}. 
	\begin{assumption}[A1]
		The action set $\cA$ is a compact set.	
	\end{assumption}

	\begin{assumption}[A2]
			$\tilde{f}\left[x_t^\alpha,a_t^\alpha,\mu_t^G;g_\alpha\right]$ and $R(x_t^{\alpha},a_t^{\alpha},\mu^G_t;g^{\alpha})$ are Lipschitz continuous in $x_t^\alpha$ and uniformly continuous with respect to $a_t^{\alpha}$.
	\end{assumption}
	
	\begin{assumption}[A3]
			The first and second derivatives of $\tilde{f}\left[x_t^\alpha,a_t^\alpha,\mu_t^G;g_\alpha\right]$ and $R(x_t^{\alpha},a_t^{\alpha},\mu^G_t;g^{\alpha})$ with respect to $x_t^\alpha$ are continuous and bounded.
	\end{assumption}
	
	\begin{assumption}[A4]
			$\tilde{f}\left[x_t^\alpha,a_t^\alpha,\mu_t^G;g_\alpha\right]$ are Lipschitz continuous in $a_t^\alpha$ and uniformly continuous with respect to $x_t^{\alpha}$.
	\end{assumption}
	
	\begin{assumption}[A5]
		For any $v\in\mathbb{R}$, $\alpha\in\left[0,1\right]$ and any probability measure ensemble $\mu_G$, the set
		\begin{align}
			S\left(x_t^\alpha, v\right)=\arg\min_{a_t^\alpha}[v\left(\tilde{f}\left[x_t^\alpha,a_t^\alpha,\mu_t^G;g_\alpha\right]\right) \\
			+ R(x_t^{\alpha},a_t^{\alpha},\mu^G_t;g^{\alpha})]
		\end{align}
			is a singleton and the resulting $a_t^\alpha$ as a function of $\left(x_t^\alpha,v\right)$ is Lipschitz continuous in $\left(x_t^\alpha,v\right)$ and uniform with respect to $\mu_t^G$ and $g_\alpha$. 
	\end{assumption}
%	
	\begin{theorem}
		Under assumptions~(A1)-(A5), there exists a solution of the fixed-point equations~\eqref{eq:m_FP} and~\eqref{eq:m_FP_ih} for every $t$.
	\end{theorem}
	
	\proof
		Under the assumption (A1)-(A5), it has been shown in~\cite{CaHu18} that there exists a solution to the \gmfg equations. Concurrently, Theorem~\ref{thm:2} and Theorem~\ref{thm:2ih} show that all \gmfe can be found using backward recursion for the finite and infinite horizon problems. This proves that under (A1)-(A5), there exists a solution of~\eqref{eq:m_FP} and~\eqref{eq:m_FP_ih} at every $t$.
	\endproof


==> Arxiv/5Numerical_example.tex <==
\label{sec:example}
In this section, we put forth a numerical example to showcase the proposed sequential decomposition in the context of a system where the relative position of the players with respect to other players in a graph affects the state of the player as well as their equilibrium strategies. We provide the following definition.
\begin{definition}
	Players $\alpha$ and $\beta$ are statistically equivalent if $\phi(\mu,\gamma,\mu^G;g^{\alpha}) = \phi^{\beta}(\mu,\gamma,\mu^G;g^{\beta})$.
\end{definition}

\begin{proposition}
	\label{prop:stat_equi}
	Mean field games with statistically equivalent players share the same mean field distribution and $\mu^G$ can be replaced by $\mu^\alpha$ for all $\alpha\in[0,1]$.
\end{proposition}

For a complete, Erdos R\'enyi, symmetric stochastic block model, and random geometric graphon, every player is statistically equivalent. Thus from proposition~\ref{prop:stat_equi}, the players share the same \mkv mean field evolution function and so the same mean field.

%\end{fact}
Let $n$ be the total number of statistically different players. Then $\mu^G$ can be replaced by $\{\mu\}_{i=1,\ldots, n}$. With the proposition we can represent the graphon mean field population state as
\begin{align}
	\mu^G &= \{\mu\}_{i=1,\ldots, n}=\mu\ \forall i
\end{align} 
\subsection{Cybersecurity Example}
%\begin{fact}

	We consider a cyber-security example where a cluster of nodes, facing a possible malware attack in a network, do a cost-benefit analysis to determine whether to opt for repairing. The results of this analysis, however, could be extended to many different cases like the vaccination in a population, entry and exit of firms, financial markets, demand response in smart-grid  and so on. The dynamics of each of the node is affected by the action of the neighboring nodes connected with different measures captured in a network graph and represented as a graphon function $G$. In this example, we assume different graphon functions and obtain the optimal policies using our sequential decomposition algorithm assuming that the graphs are symmetric with respect to the participating agents. In the model, the node can have two states $x^\alpha\in\cX=\{0,1\}$ representing healthy and infected node respectively. Similarly, there are two actions at their disposal for each of the state $a^\alpha\in\cA=\{0,1\}$ which says whether the nodes gets repaired with a cost or takes the risk by not undergoing repair. The chances of a node getting affected by a malware attack depends on the population as well as the state of the neighboring nodes according to the graphon. The dynamics of the model are given as
	\begin{align}
		x_{t+1}^\alpha = \lb {x_t^\alpha+\left(1-x_t^\alpha\right)w_t^\alpha &\text{   if } a_t^\alpha=0 \\
		0 &\text{ otherwise }}
	\end{align}
	where $w_t^\alpha\in\{0,1\}$ is a binary random variable with 
	\begin{align}
		\mP\{w_t^\alpha=1\}= \int_{\beta\in[0,1]}\sum_{x^\beta\in\cX}&f\left(x^\alpha_t,a^\alpha_t,x^\beta\right)g\left(\alpha,\beta\right)\mu_t^\beta(x^\beta)d(x^\beta)d\beta 
	\end{align}
	It is assumed that the value of $\mP\{w_t^\alpha=1\}$ is $q$ when the graph is fully connected i.e. $g\left(\alpha,\eta\right)=1$ and the mean state of the neighbors $\mu_t(x^\beta) = 1$. The value of $q$ is assumed to be $0.9$ for our simulation. The reward function is given as
	\begin{align}
		r\left(x_t^\alpha,a_t^\alpha,\mu_t\right)=-kx_t^\alpha-\lambda a_t^\alpha
	\end{align} 
	The value $k$ represents the penalty if the node gets infected and $\lambda$ represents the cost of repair. The values $k$ and $\lambda$ are assumed as $0.3$ and $0.2$ respectively for our simulation. 
	Here we implement our algorithm to derive equilibrium for this problem by considering three popular network models to capture the interaction between the population. 
	We consider the following graphons:
	\begin{enumerate}
				\item \textit{Fully Connected Graph}: The graphon function is given as
		\begin{align}
		g(\alpha,\beta)  = 1\ \forall \alpha,\beta
		\end{align}
		
		\item \textit{Erd\"os Renyi Graph}: The graphon function is given as
			\begin{align}
				g(\alpha,\beta)  = p\ \forall \alpha,\beta
			\end{align}
We assume a value $p=0.8$ for our simulation. 
		\item \textit{Stochastic Block Model}:The graphon function is given as 
			\begin{align}
				g(\alpha,\beta) = \lb {p \text{ if } \alpha,\beta\leq 0.5 \text{ or } \alpha,\beta\geq 0.5\\
				q \text{ otherwise }}
			\end{align}	
Here, $p$ represents the intra-community interaction and is assumed as $p=.9$ for our simulation. Similarly, $q=.4$ represents the inter-community interaction parameter. 	
		\item \textit{Random Geometric graph}: The graphon function is given as
		\begin{align}
			g(\alpha,\beta) = f(min(\beta-\alpha,1-\beta+\alpha))
		\end{align}
		where $f:[0,.5]\to [0,1]$ is a non-increasing function, and in our simulation we assume it to be $f(x) = e^{\frac{x}{0.5-x}}$.
	\end{enumerate}

%\begin{figure}[!htb]
%	\centering
%	\includegraphics[width=.6\textwidth]{Matlab_Code/Figures/Policy_0.eps}
%	\caption{Policy action at lower state for all graphons}
%\end{figure}



\begin{figure}[!htb]
\begin{center}
	\label{fig:policy}
	\centering
	\includegraphics[width=.6\textwidth]{Matlab_Code/Figures/Policy_1.eps}
	\caption{Policy action at higher state for all graphons}
	\end{center}
\end{figure}

%\begin{figure}[!htb]
%\centering
%\includegraphics[width=.6\textwidth]{Matlab_Code/Figures/Value_0.eps}
%\caption{Value function at lower state for all graphons}
%\end{figure}
%
%\begin{figure}[!htb]
%	\centering
%	\includegraphics[width=.6\textwidth]{Matlab_Code/Figures/Value_1.eps}
%	\caption{Value function at higher state for all graphons}
%\end{figure}

\begin{figure}[!htb]
	\label{fig:Phi}
	\centering
	\includegraphics[width=.6\textwidth]{Matlab_Code/Figures/Phi.eps}
	\centering
	\caption{Mean Field Evolution at different mean fields}
\end{figure}

\begin{figure}[!htb]
	\label{fig:mfe}
	\centering
	\includegraphics[width=.6\textwidth]{Matlab_Code/Figures/MFE.eps}
	\caption{Convergence to \glspl{gmfg} for all graphons with time}
\end{figure}

Figure~\ref{fig:policy} shows the equilibrium policy derived for different graphons for the specific cyber-security example. The policies differ as the interaction of the agents with their neighbors influences their strategies. Figure~\ref{fig:Phi} gives the relation between $\mu_t$ and $\mu_{t+1}$ as presented in the \eqref{eq:muG_update}. Figure~\ref{fig:mfe} shows the equilibrium mean field or in the specific case that we consider when with time, the a mean field distribution of $0.5$ approaches different mean field states for different graphons but with the same state dynamics.

==> Arxiv/6Conclusion.tex <==
\label{sec:Concl}
In this paper, we consider both finite and infinite horizon, large population dynamic game where each player is affected by others through a graphon mean-field population state. We present a novel backward recursive algorithm to compute non-stationary, signaling \gmfg for such games, where each player's strategy depends on its current private type and the current graphon mean-field population state. The non-triviality in the problem is that the update of population state is coupled to the strategies of the game, and is managed in the algorithm through unique construction of the fixed-point equations~\eqref{eq:m_FP},\eqref{eq:m_FP_ih}. We proved the existence of such equilibrium. Using this algorithm, we considered a malware propagation problem where we numerically computed equilibrium strategies of the players. In general, this algorithm be could instrumental in studying non-stationary equilibria in a number of applications such as financial markets, social learning, renewable energy.


==> Post_CDC/0config.tex <==
% \usepackage{bbm}
\usepackage{amsmath}
\usepackage{mathrsfs}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{amsfonts}
\usepackage[english]{babel}
% \usepackage{amsthm}
\usepackage{epstopdf}
\usepackage{dsfont}
\usepackage{hyperref}

\newtheorem{theorem}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{fact}{Fact}
\newtheorem{problem}{Problem}
\newtheorem{lemma*}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}



\newcommand{\mA}{\mathcal{A}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mN}{[N]}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cV}{\mathcal{V}}

\renewcommand{\hat}{\widehat}
\renewcommand{\bar}{\overline}
\newcommand{\ux}{\underline{x}}
\renewcommand{\star}{\ast}
\def\lpr{\left\{}
\def\rpr{\right\}}
\newcommand{\uF}{F}
\newcommand{\mP}{\mathbb{P}}
\newcommand{\mE}{\mathbb{E}}	
\newcommand\addtag{\refstepcounter{equation}\tag{\theequation}}
\newcommand{\eq}[1]{\begin{align}#1\end{align}}
\newcommand{\seq}[1]{\begin{subequations}#1\end{subequations}}

\newcommand{\lb}[1]{\left\{ \begin{array}{ll} #1 \end{array} \right.}
\newcommand*\dif{\mathop{}\!\mathrm{d}}
\newcommand{\bm}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\E}{\mathbb{E}}
 \newcommand{\nn}{\nonumber}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cZ}{\mu^G}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\tsigma}{\tilde{\sigma}}
\newcommand{\hmu}{\hat{\mu}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\tgamma}{\tilde{\gamma}}
\newcommand{\Qx}[1]{Q^{\alpha}(#1)}
\newcommand{\Qv}[1]{Q_v^{\alpha}(#1)}
\newcommand{\defeq}{\buildrel\triangle\over =}
\newcommand{\apos}{\textsc{\char13}}
\newcommand{\tred}[1]{\textcolor{red}{#1}}
\newcommand{\pushright}[1]{\ifmeasuring@ #1 \else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@ #1 \else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\newcommand{\hs}[1]{\hspace{#1}}


==> Post_CDC/0glossary.tex <==
\usepackage{xspace}
\usepackage[acronym,nogroupskip,nonumberlist,nopostdot]{glossaries}
\glsdisablehyper

% WIRELESS AND DIGITAL COMMS
\newacronym{mdp}{MDP}{Markov decision process}
\newacronym{ne}{NE}{Nash equillibrium}
\newacronym{mfe}{MFE}{mean-field equillibrium}
\newacronym{mpe}{MPE}{Markov perfect equillibrium}
\newacronym{mfg}{MFG}{mean-field game}
\newacronym{rl}{RL}{reinforcement learning}
\newacronym{marl}{MARL}{multi-agent reinforcement learning}
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{ssg}{SSG}{Stackelberg security game}
\newacronym{pse}{PSE}{perfect Stackelberg equilibrium}
\newacronym{mpse}{MPSE}{Markov \gls{pse}}
\newacronym{pomdp}{POMDP}{partially observed \gls{mdp}}
\newacronym{mc}{MC}{Monte Carlo}
\newacronym{pbe}{PBE}{perfect Bayesian equilibrium}
\newacronym{gmfg}{GMFG}{graphon mean-field game}
\newacronym{gmfe}{GMFE}{graphon mean-field equillibrium}
\newacronym{spe}{SPE}{sub-game perfect equillibrium}
\newacronym{mkv}{MKV}{McKean-Vlasov}
\newacronym{gmft}{GMFT}{graphon mean field team}


\newcommand{\mdp}{\gls{mdp}\xspace}
\newcommand{\gne}{\gls{ne}\xspace}
\newcommand{\mfe}{\gls{mfe}\xspace}
\newcommand{\mpe}{\gls{mpe}\xspace}
\newcommand{\mfg}{\gls{mfg}\xspace}
\newcommand{\mfgs}{\glspl{mfg}\xspace}
\newcommand{\rl}{\gls{rl}\xspace}
\newcommand{\marl}{\gls{marl}\xspace}
\newcommand{\ssg}{\gls{ssg}\xspace}
\newcommand{\ssgs}{\glspl{ssg}\xspace}
\newcommand{\pse}{\gls{pse}\xspace}
\newcommand{\mpse}{\gls{mpse}\xspace}
\newcommand{\pomdp}{\gls{pomdp}\xspace}
\newcommand{\pbe}{\gls{pbe}\xspace}
\newcommand{\gmfg}{\gls{gmfg}\xspace}
\newcommand{\gmfe}{\gls{gmfe}\xspace}
\newcommand{\spe}{\gls{spe}\xspace}
\newcommand{\spes}{\glspl{spe}\xspace}
\newcommand{\mkv}{\gls{mkv}\xspace}
\newcommand{\gmft}{\gls{gmft}}

==> Post_CDC/1Introduction.tex <==
Strategic interaction of interconnected agents has been an important topic of study for many decades and its relevance has been increasing rapidly with the progress of internet penetration and smartphone devices in our society. The recent decade has seen tremendous technological advancement in the field of networking applications that has led to an unprecedented scale of interaction among people and devices such as in ride sharing platforms, social media apps, cyber-physical systems, large scale renewable energy, electric vehicles, cryptocurrencies and smart grid systems. For instance, the influence of social networks in the decision making of majority of individuals is a known phenomenon. Most decisions by individuals, from which products to buy to whom to vote for, are influenced by friends and acquaintances. The emerging empirical evidence on these issues motivates the theoretical study of network effects with strategic agents. The analysis, design and control of such systems that involve strategic interactions embedded in a networked environment could lead to more intelligent and efficient applications, and can enhance our understanding of the mechanics of such interactions. 

Many of the above mentioned applications of interest have following key features: (a) large number of strategic players (b) dynamically evolving incomplete information, and (c) an underlying network. Game theory is a natural choice to model such interactions where the payoffs obtained by individuals depend on the action of her neighbors. A shortcoming of the standard approach to solve dynamic network games with incomplete information is interdependence of strategies of the players across time. Moreover, as the number of players become large as is the case in many practical scenarios considered here, computing Nash equilibrium becomes intractable. 

\subsection{Relevant Literature}

Maskin and Tirole in~\cite{MaTi01} introduced the concept of \mpe for dynamic games governed by an underlying \mdp. The strategies thus computed depend on the present state and not on the past trajectory of the game. In general, there exists a backward recursive methodology to compute \mpe of the game. Some prominent examples of the application of \mpe include~\cite{ErPa95, BeVa96, AcRo01}. Ericson and Pakes in~\cite{ErPa95} model industry dynamics for firms' entry, exit and investment participation, through a dynamic game with symmetric information, compute its \mpe, and prove ergodicity of the equilibrium process. Bergemann and V{\" a}lim{\"a}ki in~\cite{BeVa96} study a learning process in a dynamic oligopoly with strategic sellers and a single buyer, allowing for price competition among sellers. They study \mpe of the game and its convergence behavior. Acemo\u{g}lu and Robinson in~\cite{AcRo01} develop a theory of political transitions in a country by modeling it as a repeated game between the elites and the poor, and study its \mpe.

In large population games, computing \mpe with the methods specified above becomes intractable. \Glspl{mfg} were introduced by Huang, Malham\'e, and Caines in~\cite{HuMaCa06}, and Lasry and Lions in~\cite{LaLi07} to model the strategic interactions with large number of players. In such games, the individual agents have minimal impact of the overall outcome of the game and so the agents track a mean distribution of states of other agents rather than their actual states. \mfgs is an excellent and a tractable model to study large population dynamic games of incomplete information, and has been shown to be a good approximation of Nash equilibrium (or MPE) of the original game as the number of players grow large (for instance see ~\cite{Caetal15,La16,Fi17,La18,DeLaRa19} and references therein).

Parise and Ozdaglar introduced the notion of graphon games~\cite{PaOz19} to model large population \emph{static} network games, where graphon is generative model of a large random graph introduced by Lov\"asz in~\cite{Lo12}. Caines and Huang in~\cite{CaHu18} combined the ideas of \mfe and graphon games to define Graphon Mean Field Games (\glspl{gmfg}) where there are a large number of strategic agents with dynamic incomplete information who interact on an underlying fixed network generated by a known graphon. \Glspl{gmfg} combine the idea of network games defined through graphons and the mean field framework of describing multi agent homogeneous games and predicting equilibrium in a tractable manner. Large network of nodes interacting with one another can be represented as graphons and \mfgs deal with the study of such large interaction among devices and people as agents to analyze such systems to design and understand the behavior of such large scale interactions and their impact on our society. The progress in research in the mean field domain have been restricted to cases where the agents interacted in a perfect homogeneous environment and the interactions between the agents were assumed to be uniform irrespective of the location of the agent in the network. What if the population interaction was not uniform and there was a measure of how the agents interacted with each other or in other words, the payoff and the transition to the next state was conditional on the relative position of the agent in the network. The mean field distribution would be affected by it so will the optimum policies and the Nash equilibrium thus generated. The theoretical basis for such a case has been provided in~\cite{CaHu18} which generalizes the idea of \mfgs across the population with different levels of interactions through \gmfg. In this paper, we propose a sequential decomposition algorithm to compute \glspl{gmfg} by decomposing the problem across time, which reduces the complexity of computing \glspl{gmfg} from exponential to linear in time. Our algorithm can be considered as analogous to a similar decomposition algorithm provided in~\cite{Va20acc} for \mfgs, and as its extention to \glspl{gmfg}.
 
In this paper, we consider a discounted infinite horizon dynamic graphon mean field game where there is a large population of homogeneous players each having a private type. Each player sequentially makes strategic decisions and is affected by other players in its neighborhood through a graphon mean-field population state. Each player has a private type that evolves through a controlled Markov process as a function of the graphon, which only she observes and all players observe a common population state which is the distribution of other players' types. In such games, the graphon mean-field state evolves through McKean-Vlasov forward equation given a policy of the players and the graphon function. The equilibrium policy satisfies the Bellman backward equation, given the graphon mean-field states. Thus to compute equilibrium, one needs to solve the coupled backward and forward fixed-point equation in the graphon mean-field and the equilibrium policy. We further consider the case when players have a common objective and thus are a team, and provide a sequential decomposition algorithm to compute agents' optimum policies.

In order to demonstrate the utility of our algorithm to compute the \gmfe of a graphon mean field game for varying graphons, we consider a cyber-security example of malware spread problem.A cluster of nodes in a network of physical servers get infected by an independent random process. For each node, there is a higher risk of getting infected due to negative externality imposed by other infected players. A graphon function is defined that quantifies the effect of the effect of the state of other nodes in the network on the concerned node. At each time t, a node privately observes its own state and publicly observes the population of infected nodes, based on which it has to make a decision to repair or not. Upon taking an action, the transition of to the next state is governed by both its individual action and the actions affected by the neighboring agents given by a graphon function. Using our algorithm, we find equilibrium strategies of the players which are observed to be non-decreasing in the healthy population state. 

The paper is structured as follows. In Section~\ref{sec:Model}, we present a model of the graphon mean field game, followed by some preliminary result from our past research regarding \mpe in strategic dynamic games. In section ~\ref{sec:Method}, we present our main results where we present algorithm to compute \mpe for both finite and infinite horizon game, and also present existence results in~\ref{sec:Existence}. In section ~\ref{sec:Example}, we show the simulation results for the cyber-security example assuming different graphons and conclude in Section~\ref{sec:Conclusion}.

\subsection{Notation}
	We use uppercase letters for random variables and lowercase for their realizations. For any variable, subscripts represent time indices and superscripts represent player identities. We use notation $ -\alpha$ to represent all players other than player $\alpha$ i.e. $ -\alpha = \{1,2, \ldots i-1, i+1, \ldots, N \}$. We use notation $a_{t:t'}$ to represent the vector $(a_t, a_{t+1}, \ldots a_{t'})$ when $t'\geq t$ or an empty vector if $t'< t$. We use $a_t^{-\alpha}$ to mean $(a^1_t, a^2_{t}, \ldots, a_t^{i-1}, a_t^{i+1} \ldots, a^N_{t})$. We use the notation $\sum_x$ to represent both $\sum_x$ and $\int_x$, and the correct usage is determined depending on the space of $x$. We remove superscripts or subscripts if we want to represent the 
	 vector, for example $a_t$ represents $(a_t^1, \ldots, a_t^N) $. We denote the indicator function of any set $A$ by $\mathds{1}\{A\}$. For any finite set $\mathcal{S}$, $\mathcal{P}(\mathcal{S})$ represents space of probability measures on $\mathcal{S}$ and $|\mathcal{S}|$ represents its cardinality. We denote by $P^{\sigma}$ (or $E^{\sigma}$) the probability measure generated by (or expectation with respect to) strategy profile $\sigma$. We denote the set of real numbers by $\mathbb{R}$. For a probabilistic strategy profile of players $(\sigma_t^{\alpha})_{i\in [N]}$ where probability of action $a_t^{\alpha}$ conditioned on $\mu^G_{1:t},x_{1:t}^{\alpha}$ is given by $\sigma_t^{\alpha}(a_t^{\alpha}|\mu^G_{1:t},x_{1:t}^{\alpha})$, we use the short hand notation $\sigma_t^{-\alpha}(a_t^{-\alpha}|\mu^G_{1:t},x_{1:t}^{-\alpha})$ to represent $\prod_{j\neq i} \sigma_t^j(a_t^j|\mu^G_{1:t},x_{1:t}^j)$. All equalities and inequalities involving random variables are to be interpreted in \emph{a.s.} sense.


==> Post_CDC/2Model.tex <==
\subsection{Graphon Mean Field Games}
	We consider a discrete-time large population sequential game with $N$ homogeneous players with $N\to\infty$. The interactions among the $N$ players are captured in a asymptotically infinite network graph represented as a \emph{graphon}. Graphons are bounded symmetric Lebesgue measurable functions $W:\left[0,1\right]^2\to\left[0,1\right]$ which can be represented as weighted graphs on the vertex set $\left[0,1\right]$ such that $\mathbf{G}=\left\{g\left(\alpha,\beta\right):0\leq\alpha,\beta\leq 1\right\}$~\cite{CaHu18}. It is similar to an adjacency matrix defined over a $2$-dimensional plane where each entry in the matrix is the measure of coupling between the agents concerned. 
			
	At each instant $t\in[T]$, where $[T]$ represents the time horizon, a player $\alpha\in\left[0,1\right]$ observes a private type $x_t^{\alpha}\in\cX$ and commonly observes (or precomputes) the whole trajectory $\mu_{1:T}^G$, takes an action $a_t^{\alpha}\in\cA $ and receives a reward $R(x_t^{\alpha},a_t^{\alpha},\mu_t^G)$. The common observation is an ensemble of the mean field distributions with respect to all agents $\alpha\in[0,1]$ given as $\mu^G_t = \{\mu_t^{\alpha}\}_{{\alpha}\in[0,1]}$ where 	
	\begin{align}
		\mu_t^\alpha\left(x\right)=\mathds{P}\left\{x_t^\alpha=x\right\}
	\end{align}	
	with $\sum_{i=1}^{N_x} \mu^{\alpha}_t(i) = 1$. Player $\alpha$'s type evolves as a controlled Markov process,	
	\begin{align}
		\label{eqn:markov}
		x_{t+1}^{\alpha} = \tilde{f}[x_t^{\alpha} , a_t^{\alpha},  \mu_t^G; g^{\alpha} ] + w_t^{\alpha}.
	\end{align}

	The random variables $(w_t^{\alpha})_{{\alpha},t}$ are assumed to be mutually independent across players and across time. We also write the above update of $x_t^{\alpha}$ through a kernel, $x_{t+1}^{\alpha}\sim Q^{\alpha}(\cdot|x_t^{\alpha}, a_t^{\alpha}, \mu^G_t;g^{\alpha})$ which depends on the graphon function $g^\alpha=\left\{g(\alpha,\beta):0\leq\beta\leq1\right\}$. 
	
	The dynamics of the \mdp are governed both by the local information as well as the global dynamics involving the effect of the policy action of other players in the system. The idea of graphon is to capture the effect of the actions of all the other players $\beta\in[0,1]$ on player $\alpha$. In prior mean field research, it was assumed that there is a complete interaction between the players and also that these interactions were uniform. Authors in~\cite{CaHu18} provide a set of differential equations that govern such interactions in the mean field setting. The functions below show how the graphon is used in determining the effect of players on one another. The function $\tilde{f}$ in~\eqref{eqn:markov} is given as		
	\begin{align}
		\label{eq:func1}
		\tilde{f}[x_t^{\alpha} , a_t^{\alpha},  \mu_t^G; g^{\alpha} ] = f_0\left(x_t^{\alpha} , a_t^{\alpha}\right) + f\left[x_t^{\alpha} , a_t^{\alpha},  \mu_t^G; g^{\alpha} \right]
	\end{align}
	where
	\begin{align}
		\label{eq:func2}
		&f[x_t^{\alpha} , a_t^{\alpha}, \mu_t^G; g^{\alpha}] =\nn\\
			&\int_{\beta\in[0,1]}\sum_{x^\beta\in\cX}f\left(x^\alpha_t,a^\alpha_t,x^\beta\right)g\left(\alpha,\beta\right)\mu_t^\beta(x^\beta)d(x^\beta)d\beta 		
	\end{align}
	and $f_0$ represent the local effect of the agent when it takes any action and is independent of the actions taken by other agents. In the case, when the agents do not interact at all i.e. $g(\alpha,\beta)=0$, the markov process reduces only to the function $f_0$ ignoring the degenerate case when $\alpha=\beta$. 
	
	At time $t$, the player $\alpha$ observes the trajectory $(\mu^G_{1:T},x_{1:t}^{\alpha})$ and takes an action $a_t^{\alpha}$ according to a behavioral strategy $\sigma^{\alpha} = (\sigma_t^{\alpha})_t$, where $\sigma_t^{\alpha}:(\mu^G)^{T}\times\mathcal{X}^t \to \mathcal{P}(\mathcal{A})$. We denote the space of such strategies as $\mathcal{K}^{\sigma}$. This implies $A_t^{\alpha}\sim \sigma_t^{\alpha}(\cdot|\mu^G_{1:t},x_{1:t}^{\alpha})$. We denote $\mathcal{Z}^T$ to be the space of population states $\mu^G_{1:T}$ till time $T$. We denote $\mathcal{H}_t^{\alpha}=\mathcal{Z}^T \times \mathcal{X}^t$ to be the set of observed histories $(\mu^G_{1:T},x_{1:t}^{\alpha})$ of player $\alpha$.

	For finite time-horizon game, $\mathbb{G}_{T}$, each player wants to maximize its total expected discounted reward over a time horizon $T$, discounted by discount factor $0<\delta\leq1$, 
	\begin{align}
		J^{\alpha,T} :=\E^{\sigma} \left[\sum_{t=1}^T \delta^{t-1} R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha}) \right].
	\end{align} 

	For the infinite time-horizon game, $\mathbb{G}_{\infty}$, each player wants to maximize its total expected discounted reward over an infinite-time horizon discounted by a discount factor $0<\delta<1$, 
	\begin{align}
		J^{\alpha,\infty} :=\E^{\sigma} \left[\sum_{t=1}^\infty \delta^{t-1} R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha}) \right].
	\end{align} 
\subsection{Graphon Mean Field Teams}
 We  describe a model for the Graphon Mean Field Teams (\gmft s). Consider a discrete-time large population sequential game with $N$ homogeneous players with $N\to\infty$ forming a team. The interactions between these $N$ players are captured through a graphon $G$. At each instant $t\in[T]$, where $[T]$ represents the time horizon, player $\alpha$ in the team observes a private type $x_t^{\alpha}\in\cX^\alpha$ and commonly observes (or precompute) the trajectory of graphon mean fields $\mu_{1:T}^G$, takes an action $a_t^{\alpha}\in\cA^\alpha $ and receives a reward $R(x_t^{\alpha},a_t^{\alpha},\mu_t^G)$. The players choose action according to some probabilistic strategy $\sigma_t\defeq(\sigma_t^\alpha(a_t^\alpha\vert x_t^\alpha,\mu_t^G;g^\alpha))_{\alpha\in[0,1]}$ and the process $\{X_t^{\alpha}\}_t$ evolves for each player $\alpha$ as a conditionally independent Markov processes as was expressed in~\eqref{eq:func1} and~\eqref{eq:func2}. The cumulative reward can be expressed as
	\begin{align}
		R_c[a_t,& \mu_t^G; g] =\int_{\alpha}\sum_{x^\alpha\in\cX}\int_{\beta}\sum_{x^\beta\in\cX}R^\prime d\beta d\alpha
	\end{align}
	where
	\begin{align}
		R^\prime= R\left(x^\alpha,a^\alpha_t,x^\beta\right)g\left(\alpha,\beta\right)&\mu_t^\beta(x^\beta)\mu_t^\alpha(x^\alpha)
	\end{align}
	
\subsection{Solution concepts: NE and \gmfe}
	The Nash equilibrium (NE) of $\mathbb{G}_{T}$ is defined as strategies $\tsigma = (\tsigma_t^{\alpha})_{\alpha\in\left[0,1\right],t\in\left[T\right]}$ that satisfy, for all $\alpha\in\left[0,1\right]$, 
	\begin{align}
		\E^{\tsigma^{\alpha},\tsigma^{-\alpha}}&\left[\sum_{t=1}^T \delta^{t-1} R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha}) \right]\nn\\
		&\geq \E^{\sigma^{\alpha},\tsigma^{-\alpha}}\left[\sum_{t=1}^T \delta^{t-1} R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha})\right],
	\end{align} 
	For graphon mean field games, \gmfe is defined in~\cite{}, which we use in this paper. It is shown that \gmfe is limit of NE as number of players grow to infinity. A \gmfe $(\tsigma)$ satisfies sequential rationality such that for $\mathbb{G}_T$, $\forall\alpha\in\left[0,1\right], t \in \left[T\right], h^{\alpha}_t \in \cH^{\alpha}_t, {\sigma^{\alpha}}$,
	\begin{align}
		&\E^{\tsigma^{\alpha}}\left[\sum_{n=t}^T\delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:T},x_{1:t}^{\alpha}\right]\nn\\
			&\geq\E^{{\sigma}^{\alpha}}\left[\sum_{n=t}^T \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:T},x_{1:t}^{\alpha}\right]  \label{eq:seqeq2}
	\end{align}
	where given the \gmfe strategies $\tsigma$ the mean fields evolve through the Fokker-Planck-Kolmogorov equation
	\eq{
	....
	}
	NE and \gmfe for $\mathbb{G}_{\infty}$ are defined in a similar way where summation in the above equations is taken such that $T$ is replaced by $\infty$.
	
	For the team problem, an optimum \gmft  policy is defined as ...

==> Post_CDC/3Method.tex <==
In this section, we will provide a backward recursive methodology to compute \glspl{gmfe} for both $\mathbb{G}_{T}$ and $\mathbb{G}_{\infty}$. We will consider Markovian equilibrium strategies of player $\alpha$ which depend on the common information at time $t$, $\mu^G_{t}$, and on its current type $x_t^{\alpha}$.\footnote{Note however, that the unilateral deviations of the player are considered in the space of all strategies.}  Equivalently, player $\alpha$ takes action of the form $A_t^{\alpha}\sim \sigma_t^{\alpha}(\cdot|\mu^G_t,x_t^{\alpha})$. Similar to the common agent approach in~\cite{NaMaTe13}, an alternate and equivalent way of defining the strategies of the players is as follows. We first generate partial function $\gamma_t^{\alpha}:\cX\to\cP(\cA)$ as a function of $\mu^G_t$ through an equilibrium generating function $\theta_t^{\alpha}:\cZ\to(\cX\to\cP(\cA))$ such that $\gamma_t^{\alpha} = \theta_t^{\alpha}[\mu^G_t]$. Then action $A_t^{\alpha}$ is generated by applying this prescription function $\gamma_t^{\alpha}$ on player $\alpha$'s current private information $x_t^{\alpha}$, i.e. $A_t^{\alpha}\sim \gamma_t^{\alpha}(\cdot|x_t^{\alpha})$. Thus $A_t^{\alpha}\sim \sigma_t^{\alpha}(\cdot|\mu^G_{t},x_t^{\alpha}) = \theta_t^{\alpha}[\mu^G_t](\cdot|x_t^{\alpha})$.
	
For a given prescription function $\gamma^{\alpha}_t = \theta^{\alpha}[\mu^G_t]$, the graphon mean-field $\mu^G_t$ evolves according to the discrete-time McKean Vlasov equation, $\forall y\in\cX$ and $\forall \alpha\in[0,1]$:
\begin{align}
	\mu^{\alpha}_{t+1}(y) =\sum_{x\in\cX}\sum_{a\in \cA} \mu^{\alpha}_t(x)\gamma^{\alpha}_t(a|x)Q\left(y|x,a,\mu^G_t;g^{\alpha}\right), \label{eq:muG_update}
\end{align}
which implies
\begin{align}
	\mu^{\alpha}_{t+1}&= \phi(\mu^{\alpha}_t,\gamma^{\alpha}_t,\mu^G_t;g^{\alpha})\\
	\mu_{t+1}^G &= \phi(\mu_t^G,\gamma_t;g^{\alpha}) 
\end{align}

\subsection{Backward recursive algorithm for $\mathbb{G}_{T}$} \label{sec:fhbr1}
	In this subsection, we will provide a methodology to generate \gmfe of $\mathbb{G}_{T}$ of the form described above. We define an equilibrium generating function $(\theta_t)_{t\in[T]}$, where $\theta_t:\cZ\to\{\cX\to\mathcal{P}(\cA) \}$, where for each $\mu^G_t $, we generate $\tgamma_t = \theta_t[\mu^G_t]$. In addition, we generate a reward-to-go function $(V^{\alpha}_t)_{t\in[T]}$, where $V^{\alpha}_t:\cZ\times\cX\to\mathbb{R}$. These quantities are generated through a fixed-point equation as follows.
	\begin{enumerate}
		\item Initialize $\forall \mu^G_{T+1}, x_{T+1}^{\alpha}\in \cX$,
		\begin{align}
			V^{\alpha}_{T+1}(\mu^G_{T+1},x_{T+1}^{\alpha}) \defeq 0.   \label{eq:VT+1}
		\end{align}

		\item For $t = T,T-1, \ldots 1, \ \forall \mu^G_t$, let $\theta_t[\mu^G_t] $ be generated as follows. Set $\tilde{\gamma}_t = \theta_t[\mu^G_t]$, where $\tilde{\gamma}_t$ is the solution of the following fixed-point equation\footnote{We discuss the existence of solution of this fixed-point equation in Section~\ref{sec:Existence}}, $\forall i \in [N],x_t^{\alpha}\in \cX$,
		\begin{align}
				\tilde{\gamma}_t(\cdot|x_t^{\alpha}) \in  &\arg\max_{\gamma_t(\cdot|x_t^{\alpha})} \E^{\gamma_t(\cdot|x_t^{\alpha})}[ R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha})+\nn\\
				&\delta V^{\alpha}_{t+1}(\phi(\mu^G_t,\tgamma_t;g^{\alpha}), X_{t+1}^{\alpha}) | \mu^G_t,x_t^{\alpha}] , \label{eq:m_FP}
		\end{align}
		where expectation in \eqref{eq:m_FP} is with respect to random variable $(A_t^{\alpha},X_{t+1}^{\alpha})$ through the probability measure $\gamma_t(a_t^{\alpha}|x_t^{\alpha})Q^{\alpha}(x_{t+1}^{\alpha}|x_t^{\alpha},a_t^{\alpha},\mu^G_t;g^{\alpha})$. We note that the solution of~\eqref{eq:m_FP}, $\tgamma_t$, appears both on the left of~\eqref{eq:m_FP} and on the right side in the update of $\mu^G_t$, and is thus unlike the fixed-point equation found in Bayesian Nash equilibrium.

		Furthermore, using the quantity $\tilde{\gamma}_t$ found above, define
		\begin{align}
			V^{\alpha}_{t}(\mu^G_t,x_t^{\alpha})&\defeq\E^{\tilde{\gamma}_t(\cdot|x^{\alpha})}[R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha})+\nn\\
			&\delta V^{\alpha}_{t+1}(\phi(\mu^G_t,\tgamma_t), X_{t+1}^{\alpha}) | \mu^G_t,x_t^{\alpha}].  \label{eq:Vdef}
		\end{align}
	\end{enumerate}
	Then, an equilibrium strategy is defined as 
	\begin{align}
		\tilde{\sigma}_t^{\alpha}(a_t^{\alpha}|\mu^G_{1:t},x_{1:t}^{\alpha}) = \tilde{\gamma}_t(a_t^{\alpha}|x_t^{\alpha}), \label{eq:sigma_fh}
	\end{align}
	where $\tilde{\gamma}_t = \theta[\mu^G_t]$. 

	In the following theorem, we show that the strategy thus constructed is a \glspl{gmfg} of the game.

%%%%%%%%%%%%%
	\begin{theorem}
	\label{Thm:Main}
		A strategy $(\tsigma)$ constructed from the above algorithm is a \gmfe of the game i.e. $\forall t, h^{\alpha}_t \in \cH^{\alpha}_t, {\sigma^{\alpha}}$,
		\begin{align}
			\label{eq:prop}
			&\E^{(\tsigma^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^T \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] \geq \nn\\
			&\E^{({\sigma}^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^T \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] 
		\end{align}
	\end{theorem}
	\begin{proof}
		Please refer to the online version for proofs.
	\end{proof}

\subsection{Converse}
	In the following, we show that every \gmfe can be found using the above backward recursion.

	\begin{theorem}[Converse]
	\label{thm:2}
		Let $\tsigma$ be a \gmfe of the graphon mean field game. Then there exists an equilibrium generating function $\theta$ that satisfies \eqref{eq:m_FP} in backward recursion such that  $\tsigma$ is defined using $\theta$.
	\end{theorem}
	\begin{proof}
		Please refer to the online version for proofs.
	\end{proof}

\subsection{Backward recursive algorithm for $\mathbb{G}_{\infty}$} \label{sec:fhbr}
	In this section, we consider the infinite-horizon problem $\mathbb{G}_{\infty}$, for which we assume the reward function $R$ to be absolutely bounded.

	We define an equilibrium generating function $\theta:\cZ\to\{\cX\to\mathcal{P}(\cA) \}$, where for each $\mu^G_t $, we generate $\tgamma_t = \theta[\mu^G_t]$. In addition, we generate a reward-to-go function $V:\cZ\times\cX\to\mathbb{R}$.
	These quantities are generated through a fixed-point equation as follows.

	For all $\mu^G,$ set $\tilde{\gamma} = \theta[z]$. Then $(\tilde{\gamma},V)$ are solution of the following fixed-point equation\footnote{We discuss the existence of solution of this fixed-point equation in Section~\ref{sec:Existence}}, $\forall z\in\cZ,x^{\alpha}\in \cX$,
	\begin{align}
		\label{eq:m_FP_ih}
		\tilde{\gamma}(\cdot|x^{\alpha}) \in \arg\max_{\gamma(\cdot|x^{\alpha})}&\E^{\gamma(\cdot|x^{\alpha})} [R(x^{\alpha},A^{\alpha},\mu^G;g^{\alpha})+\nn\\
		&\delta V(\phi(z,\tgamma), X^{{\alpha}'};g^{\alpha}) | \mu^G,x^{\alpha}] ,
	\end{align}		
	\begin{align}
		V(z,x^{\alpha}) =\  &\E^{\tilde{\gamma}(\cdot|x^{\alpha})} [ R(x^{\alpha},A^{\alpha},\mu^G;g^{\alpha})+\nn\\
		&\delta V (\phi(\mu^G,\tgamma;g^{\alpha}), X^{{\alpha}'})\vert \mu^G,x^{\alpha}]. 
	\end{align}
	where expectation in \eqref{eq:m_FP_ih} is with respect to random variable $(A^{\alpha},X^{{\alpha},\prime})$ through the measure $\gamma(a^{\alpha}|x^{\alpha})Q^{\alpha}(x^{{\alpha}'}|x^{\alpha},a^{\alpha},\mu^G)$.

	Then an equilibrium strategy is defined as 
	\begin{align}
		\tilde{\sigma}^{\alpha}(a_t^{\alpha}|\mu^G_{1:t},x_{1:t}^{\alpha}) = \tilde{\gamma}(a_t^{\alpha}|x_t^{\alpha}), \label{eq:sigma_ih}
	\end{align}
	where $\tilde{\gamma} = \theta[\mu^G_t]$.

	The following theorem shows that the strategy thus constructed is a \gmfe of the game.

	\begin{theorem}
	\label{thih}
		A strategy $(\tsigma)$ constructed from the above algorithm is a \gmfe of the game i.e. $\forall t, h^{\alpha}_t \in \cH^{\alpha}_t, {\sigma^{\alpha}}$,

		\begin{align}
			\label{eq:prop_ih}
			&\E^{(\tsigma^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^\infty \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] \geq\nn\\
			&\E^{({\sigma}^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^\infty \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right], 
		\end{align} 
	\end{theorem}
	\begin{proof}
		Please refer to the online version for proofs.
	\end{proof}

\subsection{Converse}
	In the following, we show that every \gmfe can be found using the above backward recursion.
	\begin{theorem}[Converse]
	\label{thm:2ih}
		Let $\tsigma$ be a \gmfe the graphon mean field game. Then there exists an equilibrium generating function $\theta$	that satisfies \eqref{eq:m_FP} in backward recursion such that  $\tsigma$ is defined using $\theta$.
	\end{theorem}
	\begin{proof}
		Please refer to the online version for the proofs.
	\end{proof}

\subsection{Backward recursive algorithm for \gmft}

In this subsection, we will provide a methodology to generate optimal control policy for coupled teams with mean field sharing. We define an optimal policy $(\theta_t)_{t\in[T]}$, where $\theta_t:\cZ\to\times_{\alpha\in[0,1]}\{\cX^\alpha\to\mathcal{P}(\cA^\alpha) \}^\alpha$, where for each $\mu^G_t $, we generate $\tgamma_t = \theta_t[\mu^G_t]$ and $\tgamma_t = (\tgamma^\alpha_t)_{\alpha\in[0,1]}$. In addition, we generate a reward-to-go function $(V_t)_{t\in[T]}$, where $V_t:\cZ\to\mathbb{R}$. These quantities are generated as follows.
	\begin{enumerate}
		\item Initialize $\forall \mu^G_{T+1}\in \cX$,
		\begin{align}
			V_{T+1}(\mu^G_{T+1}) \defeq 0.   \label{eq:VT1+1}
		\end{align}

		\item For $t = T,T-1, \ldots 1, \ \forall \mu^G_t$, let $\theta_t[\mu^G_t] $ be generated as follows. Set $\tilde{\gamma}_t = \theta_t[\mu^G_t]$, where $\tilde{\gamma}_t$. $\forall i \in [N]$,
		\begin{align}
				\tilde{\gamma}_t \in  &\arg\max_{\gamma_t} \E^{\gamma_t,\mu_t^G}[ R_c(A_t,\mu^G_t;g)+\nn\\
				&\delta V_{t+1}(\phi(\mu^G_t,\gamma_t;g)) | \mu^G_t] , \label{eq:m_FP1}
		\end{align}
		where expectation in \eqref{eq:m_FP1} is with respect to random variable $(A_t)$ through the probability measure $\left(\gamma_t^\alpha\left(a^\alpha_t\vert x_t^\alpha\right)\mu^\alpha_t\left(x_t^\alpha\right)\right)_{\alpha\in[0,1]}$.

		Furthermore, using the quantity $\tilde{\gamma}_t$ found above, define
		\begin{align}
			V_{t}(\mu^G_t)&\defeq\E^{\tilde{\gamma}_t, \mu^G_t}[R_c(A_t,\mu^G_t;g)+\nn\\
			&\delta V_{t+1}(\phi(\mu^G_t,\tgamma_t)) | \mu^G_t].  \label{eq:Vdef1}
		\end{align}
	\end{enumerate}
	Then, an optimlal strategy is defined as 
	\begin{align}
		\tilde{\sigma}_t(a_t|\mu^G_{1:t}) = \tilde{\gamma}_t, \label{eq:sigma_fh1}
	\end{align}
	where $\tilde{\gamma}_t = \theta[\mu^G_t]$. 
	The following theorem shows that the strategy thus constructed is optimal.
	\begin{theorem}
	\label{thih1}
		A strategy $(\tsigma)$ constructed from the above algorithm is team optimal i.e. $\forall t, h_t \in \cH_t, {\sigma}$,

		\begin{align}
			\label{eq:prop_ih1}
			&\E^{\tsigma}\left[\sum_{n=t}^\infty \delta^{n-t} R_c(A_n,\mu^G_n;g)|\mu^G_{1:t}\right] \geq\nn\\
			&\E^{({\sigma} \tsigma)}\left[\sum_{n=t}^\infty \delta^{n-t} R(X_n,A_n,\mu^G_n;g)|\mu^G_{1:t}\right], 
		\end{align} 
	\end{theorem}
	\begin{proof}
		The process $\{\mu^G_t,\gamma_t \}_t$ is a controlled Markov process since.... Thus above result follows from the theory of Markov decision processes.
	\end{proof}

==> Post_CDC/4Existence.tex <==
\label{sec:exists}
	In this section, we discuss sufficient conditions for the existence of a solution of the fixed-point equations~\eqref{eq:m_FP} and~\eqref{eq:m_FP_ih}. 
	\begin{assumption}[A1]
		The action set $\cA$ is a compact set.	
	\end{assumption}

	\begin{assumption}[A2]
		$\tilde{f}\left[x_t^\alpha,a_t^\alpha,\mu_t^G;g_\alpha\right]$ and $R(x_t^{\alpha},a_t^{\alpha},\mu^G_t;g^{\alpha})$ are Lipschitz continuous in $x_t^\alpha$ and uniformly continuous with respect to $a_t^{\alpha}$.
	\end{assumption}
	
	\begin{assumption}[A3]
			The first and second derivatives of $\tilde{f}\left[x_t^\alpha,a_t^\alpha,\mu_t^G;g_\alpha\right]$ and $R(x_t^{\alpha},a_t^{\alpha},\mu^G_t;g^{\alpha})$ with respect to $x_t^\alpha$ are continuous and bounded.
	\end{assumption}
	
	\begin{assumption}[A4]
			$\tilde{f}\left[x_t^\alpha,a_t^\alpha,\mu_t^G;g_\alpha\right]$ are Lipschitz continuous in $a_t^\alpha$ and uniformly continuous with respect to $x_t^{\alpha}$.
	\end{assumption}
	
	\begin{assumption}[A5]
		For any $v\in\mathbb{R}$, $\alpha\in\left[0,1\right]$ and any probability measure ensemble $\mu_G$, the set
		\begin{align}
			S\left(x_t^\alpha, v\right)=\arg\min_{a_t^\alpha}[v\left(\tilde{f}\left[x_t^\alpha,a_t^\alpha,\mu_t^G;g_\alpha\right]\right) \\
			+ R(x_t^{\alpha},a_t^{\alpha},\mu^G_t;g^{\alpha})]
		\end{align}
			is a singleton and the resulting $a_t^\alpha$ as a function of $\left(x_t^\alpha,v\right)$ is Lipschitz continuous in $\left(x_t^\alpha,v\right)$ and uniform with respect to $\mu_t^G$ and $g_\alpha$. 
	\end{assumption}
%	
	\begin{theorem}
		Under assumptions~(A1)-(A5), there exists a solution of the fixed-point equations~\eqref{eq:m_FP} and~\eqref{eq:m_FP_ih} for every $t$.
	\end{theorem}
	
	\proof
		Under the assumption (A1)-(A5), it has been shown in~\cite{CaHu18} that there exists a solution to the \gmfg equations. Concurrently, Theorem~\ref{thm:2} and Theorem~\ref{thm:2ih} show that all \gmfe can be found using backward recursion for the finite and infinite horizon problems. This proves that under (A1)-(A5), there exists a solution of~\eqref{eq:m_FP} and~\eqref{eq:m_FP_ih} at every $t$.
	\endproof


==> Post_CDC/5Numerical_example.tex <==
\label{sec:example}
In this section, we put forth a numerical example to showcase the proposed sequential decomposition in the context of a system where the relative position of the players with respect to other players in a graph affects the state of the player as well as their equilibrium strategies. We provide the following definition.
\begin{definition}
	Players $\alpha$ and $\beta$ are statistically equivalent if $\phi(\mu,\gamma,\mu^G;g^{\alpha}) = \phi^{\beta}(\mu,\gamma,\mu^G;g^{\beta})$.
\end{definition}

\begin{proposition}
	\label{prop:stat_equi}
	Mean field games with statistically equivalent players share the same mean field distribution and $\mu^G$ can be replaced by $\mu^\alpha$ for all $\alpha\in[0,1]$.
\end{proposition}

For a complete, Erdos R\'enyi, symmetric stochastic block model, and random geometric graphon, every player is statistically equivalent. Thus from proposition~\ref{prop:stat_equi}, the players share the same \mkv mean field evolution function and so the same mean field.

%\end{fact}
Let $n$ be the total number of statistically different players. Then $\mu^G$ can be replaced by $\{\mu\}_{i=1,\ldots, n}$. With the proposition we can represent the graphon mean field population state as
\begin{align}
	\mu^G &= \{\mu\}_{i=1,\ldots, n}=\mu\ \forall i
\end{align} 
\subsection{Cybersecurity Example}
%\begin{fact}

	We consider a cyber-security example where a cluster of nodes, facing a possible malware attack in a network, do a cost-benefit analysis to determine whether to opt for repairing. The results of this analysis, however, could be extended to many different cases like the vaccination in a population, entry and exit of firms, financial markets, demand response in smart-grid  and so on. The dynamics of each of the node is affected by the action of the neighboring nodes connected with different measures captured in a network graph and represented as a graphon function $G$. In this example, we assume different graphon functions and obtain the optimal policies using our sequential decomposition algorithm assuming that the graphs are symmetric with respect to the participating agents. In the model, the node can have two states $x^\alpha\in\cX=\{0,1\}$ representing healthy and infected node respectively. Similarly, there are two actions at their disposal for each of the state $a^\alpha\in\cA=\{0,1\}$ which says whether the nodes gets repaired with a cost or takes the risk by not undergoing repair. The chances of a node getting affected by a malware attack depends on the population as well as the state of the neighboring nodes according to the graphon. The dynamics of the model are given as
	\begin{align}
		x_{t+1}^\alpha = \lb {x_t^\alpha+\left(1-x_t^\alpha\right)w_t^\alpha &\text{   if } a_t^\alpha=0 \\
		0 &\text{ otherwise }}
	\end{align}
	where $w_t^\alpha\in\{0,1\}$ is a binary random variable with 
	\begin{align}
		&\mP\{w_t^\alpha=1\}=\nn\\
		 &\int_{\beta\in[0,1]}\sum_{x^\beta\in\cX}&f\left(x^\alpha_t,a^\alpha_t,x^\beta\right)g\left(\alpha,\beta\right)\mu_t^\beta(x^\beta)d(x^\beta)d\beta 
	\end{align}
	It is assumed that the value of $\mP\{w_t^\alpha=1\}$ is $q$ when the graph is fully connected i.e. $g\left(\alpha,\eta\right)=1$ and the mean state of the neighbors $\mu_t(x^\beta) = 1$. The value of $q$ is assumed to be $0.9$ for our simulation. The reward function is given as
	\begin{align}
		r\left(x_t^\alpha,a_t^\alpha,\mu_t\right)=-kx_t^\alpha-\lambda a_t^\alpha
	\end{align} 
	The value $k$ represents the penalty if the node gets infected and $\lambda$ represents the cost of repair. The values $k$ and $\lambda$ are assumed as $0.3$ and $0.2$ respectively for our simulation. 
	Here we implement our algorithm to derive equilibrium for this problem by considering three popular network models to capture the interaction between the population. 
	We consider the following graphons:
	\begin{enumerate}
				\item \textit{Fully Connected Graph}: The graphon function is given as
		\begin{align}
		g(\alpha,\beta)  = 1\ \forall \alpha,\beta
		\end{align}
		
		\item \textit{Erd\"os Renyi Graph}: The graphon function is given as
			\begin{align}
				g(\alpha,\beta)  = p\ \forall \alpha,\beta
			\end{align}
We assume a value $p=0.8$ for our simulation. 
		\item \textit{Stochastic Block Model}:The graphon function is given as 
			\begin{align}
				g(\alpha,\beta) = \lb {p \text{ if } \alpha,\beta\leq 0.5 \text{ or } \alpha,\beta\geq 0.5\\
				q \text{ otherwise }}
			\end{align}	
Here, $p$ represents the intra-community interaction and is assumed as $p=.9$ for our simulation. Similarly, $q=.4$ represents the inter-community interaction parameter. 	
		\item \textit{Random Geometric graph}: The graphon function is given as
		\begin{align}
			g(\alpha,\beta) = f(min(\beta-\alpha,1-\beta+\alpha))
		\end{align}
		where $f:[0,.5]\to [0,1]$ is a non-increasing function, and in our simulation we assume it to be $f(x) = e^{\frac{x}{0.5-x}}$.
	\end{enumerate}

%\begin{figure}[!htb]
%	\centering
%	\includegraphics[width=.6\textwidth]{Matlab_Code/Figures/Policy_0.eps}
%	\caption{Policy action at lower state for all graphons}
%\end{figure}



\begin{figure}[!htb]
\begin{center}
	\label{fig:policy}
	\centering
	\includegraphics[width=.4\textwidth]{Policy_1.pdf}
	\caption{Policy action at higher state for all graphons}
	\end{center}
\end{figure}

%\begin{figure}[!htb]
%\centering
%\includegraphics[width=.6\textwidth]{Matlab_Code/Figures/Value_0.eps}
%\caption{Value function at lower state for all graphons}
%\end{figure}
%
%\begin{figure}[!htb]
%	\centering
%	\includegraphics[width=.6\textwidth]{Matlab_Code/Figures/Value_1.eps}
%	\caption{Value function at higher state for all graphons}
%\end{figure}

\begin{figure}[!htb]
	\label{fig:Phi}
	\centering
	\includegraphics[width=.4\textwidth]{Phi.pdf}
	\centering
	\caption{Mean Field Evolution at different mean fields}
\end{figure}

\begin{figure}[!htb]
	\label{fig:mfe}
	\centering
	\includegraphics[width=.4\textwidth]{MFE.pdf}
	\caption{Convergence to \glspl{gmfg} for all graphons with time}
\end{figure}

Figure~\ref{fig:policy} shows the equilibrium policy derived for different graphons for the specific cyber-security example. The policies differ as the interaction of the agents with their neighbors influences their strategies. Figure~\ref{fig:Phi} gives the relation between $\mu_t$ and $\mu_{t+1}$ as presented in the \eqref{eq:muG_update}. Figure~\ref{fig:mfe} shows the equilibrium mean field or in the specific case that we consider when with time, the a mean field distribution of $0.5$ approaches different mean field states for different graphons but with the same state dynamics. [Add similar diagrams for the team problem. Also comment on the structure of the policies (and maybe value functions also?)]

==> Post_CDC/6Conclusion.tex <==
\label{sec:Concl}
In this paper, we consider both finite and infinite horizon, large population dynamic game where each player is affected by others through a graphon mean-field population state. We present a novel backward recursive algorithm to compute non-stationary, signaling \gmfg for such games, where each player's strategy depends on its current private type and the current graphon mean-field population state. The non-triviality in the problem is that the update of population state is coupled to the strategies of the game, and is managed in the algorithm through unique construction of the fixed-point equations~\eqref{eq:m_FP},\eqref{eq:m_FP_ih}. We proved the existence of such equilibrium. Using this algorithm, we considered a malware propagation problem where we numerically computed equilibrium strategies of the players. In general, this algorithm be could instrumental in studying non-stationary equilibria in a number of applications such as financial markets, social learning, renewable energy.


==> Post_CDC/__latexindent_temp.tex <==
In this section, we will provide a backward recursive methodology to compute \glspl{gmfg} for both $\mathbb{G}_{T}$ and $\mathbb{G}_{\infty}$. We will consider Markovian equilibrium strategies of player $\alpha$ which depend on the common information at time $t$, $\mu^G_{t}$, and on its current type $x_t^{\alpha}$.\footnote{Note however, that the unilateral deviations of the player are considered in the space of all strategies.}  Equivalently, player $\alpha$ takes action of the form $A_t^{\alpha}\sim \sigma_t^{\alpha}(\cdot|\mu^G_t,x_t^{\alpha})$. Similar to the common agent approach in~\cite{NaMaTe13}, an alternate and equivalent way of defining the strategies of the players is as follows. We first generate partial function $\gamma_t^{\alpha}:\cX\to\cP(\cA)$ as a function of $\mu^G_t$ through an equilibrium generating function $\theta_t^{\alpha}:\cZ\to(\cX\to\cP(\cA))$ such that $\gamma_t^{\alpha} = \theta_t^{\alpha}[\mu^G_t]$. Then action $A_t^{\alpha}$ is generated by applying this prescription function $\gamma_t^{\alpha}$ on player $\alpha$'s current private information $x_t^{\alpha}$, i.e. $A_t^{\alpha}\sim \gamma_t^{\alpha}(\cdot|x_t^{\alpha})$. Thus $A_t^{\alpha}\sim \sigma_t^{\alpha}(\cdot|\mu^G_{t},x_t^{\alpha}) = \theta_t^{\alpha}[\mu^G_t](\cdot|x_t^{\alpha})$.
	
For a given prescription function $\gamma^{\alpha}_t = \theta^{\alpha}[\mu^G_t]$, the graphon mean-field $\mu^G_t$ evolves according to the discrete-time McKean Vlasov equation, $\forall y\in\cX$ and $\forall \alpha\in[0,1]$:
\begin{align}
	\mu^{\alpha}_{t+1}(y) =\sum_{x\in\cX}\sum_{a\in \cA} \mu^{\alpha}_t(x)\gamma^{\alpha}_t(a|x)Q\left(y|x,a,\mu^G_t;g^{\alpha}\right), \label{eq:muG_update}
\end{align}
which implies
\begin{align}
	\mu^{\alpha}_{t+1}&= \phi(\mu^{\alpha}_t,\gamma^{\alpha}_t,\mu^G_t;g^{\alpha})\\
	\mu_{t+1}^G &= \phi(\mu_t^G,\gamma_t;g^{\alpha}) 
\end{align}

\subsection{Backward recursive algorithm for $\mathbb{G}_{T}$} \label{sec:fhbr1}
	In this subsection, we will provide a methodology to generate \gmfe of $\mathbb{G}_{T}$ of the form described above. We define an equilibrium generating function $(\theta_t)_{t\in[T]}$, where $\theta_t:\cZ\to\{\cX\to\mathcal{P}(\cA) \}$, where for each $\mu^G_t $, we generate $\tgamma_t = \theta_t[\mu^G_t]$. In addition, we generate a reward-to-go function $(V^{\alpha}_t)_{t\in[T]}$, where $V^{\alpha}_t:\cZ\times\cX\to\mathbb{R}$. These quantities are generated through a fixed-point equation as follows.
	\begin{enumerate}
		\item Initialize $\forall \mu^G_{T+1}, x_{T+1}^{\alpha}\in \cX$,
		\begin{align}
			V^{\alpha}_{T+1}(\mu^G_{T+1},x_{T+1}^{\alpha}) \defeq 0.   \label{eq:VT+1}
		\end{align}

		\item For $t = T,T-1, \ldots 1, \ \forall \mu^G_t$, let $\theta_t[\mu^G_t] $ be generated as follows. Set $\tilde{\gamma}_t = \theta_t[\mu^G_t]$, where $\tilde{\gamma}_t$ is the solution of the following fixed-point equation\footnote{We discuss the existence of solution of this fixed-point equation in Section~\ref{sec:Existence}}, $\forall i \in [N],x_t^{\alpha}\in \cX$,
		\begin{align}
				\tilde{\gamma}_t(\cdot|x_t^{\alpha}) \in  &\arg\max_{\gamma_t(\cdot|x_t^{\alpha})} \E^{\gamma_t(\cdot|x_t^{\alpha})}[ R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha})+\nn\\
				&\delta V^{\alpha}_{t+1}(\phi(\mu^G_t,\tgamma_t;g^{\alpha}), X_{t+1}^{\alpha}) | \mu^G_t,x_t^{\alpha}] , \label{eq:m_FP}
		\end{align}
		where expectation in \eqref{eq:m_FP} is with respect to random variable $(A_t^{\alpha},X_{t+1}^{\alpha})$ through the probability measure $\gamma_t(a_t^{\alpha}|x_t^{\alpha})Q^{\alpha}(x_{t+1}^{\alpha}|x_t^{\alpha},a_t^{\alpha},\mu^G_t;g^{\alpha})$. We note that the solution of~\eqref{eq:m_FP}, $\tgamma_t$, appears both on the left of~\eqref{eq:m_FP} and on the right side in the update of $\mu^G_t$, and is thus unlike the fixed-point equation found in Bayesian Nash equilibrium.

		Furthermore, using the quantity $\tilde{\gamma}_t$ found above, define
		\begin{align}
			V^{\alpha}_{t}(\mu^G_t,x_t^{\alpha})&\defeq\E^{\tilde{\gamma}_t(\cdot|x^{\alpha})}[R(X_t^{\alpha},A_t^{\alpha},\mu^G_t;g^{\alpha})+\nn\\
			&\delta V^{\alpha}_{t+1}(\phi(\mu^G_t,\tgamma_t), X_{t+1}^{\alpha}) | \mu^G_t,x_t^{\alpha}].  \label{eq:Vdef}
		\end{align}
	\end{enumerate}
	Then, an equilibrium strategy is defined as 
	\begin{align}
		\tilde{\sigma}_t^{\alpha}(a_t^{\alpha}|\mu^G_{1:t},x_{1:t}^{\alpha}) = \tilde{\gamma}_t(a_t^{\alpha}|x_t^{\alpha}), \label{eq:sigma_fh}
	\end{align}
	where $\tilde{\gamma}_t = \theta[\mu^G_t]$. 

	In the following theorem, we show that the strategy thus constructed is a \glspl{gmfg} of the game.

%%%%%%%%%%%%%
	\begin{theorem}
	\label{Thm:Main}
		A strategy $(\tsigma)$ constructed from the above algorithm is a \gmfe of the game i.e. $\forall t, h^{\alpha}_t \in \cH^{\alpha}_t, {\sigma^{\alpha}}$,
		\begin{align}
			\label{eq:prop}
			&\E^{(\tsigma^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^T \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] \geq \nn\\
			&\E^{({\sigma}^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^T \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] 
		\end{align}
	\end{theorem}
	\begin{proof}
		Please refer to the online version for proofs.
	\end{proof}

\subsection{Converse}
	In the following, we show that every \gmfe can be found using the above backward recursion.

	\begin{theorem}[Converse]
	\label{thm:2}
		Let $\tsigma$ be a \gmfe of the graphon mean field game. Then there exists an equilibrium generating function $\theta$ that satisfies \eqref{eq:m_FP} in backward recursion such that  $\tsigma$ is defined using $\theta$.
	\end{theorem}
	\begin{proof}
		Please refer to the online version for proofs.
	\end{proof}

\subsection{Backward recursive algorithm for $\mathbb{G}_{\infty}$} \label{sec:fhbr}
	In this section, we consider the infinite-horizon problem $\mathbb{G}_{\infty}$, for which we assume the reward function $R$ to be absolutely bounded.

	We define an equilibrium generating function $\theta:\cZ\to\{\cX\to\mathcal{P}(\cA) \}$, where for each $\mu^G_t $, we generate $\tgamma_t = \theta[\mu^G_t]$. In addition, we generate a reward-to-go function $V:\cZ\times\cX\to\mathbb{R}$.
	These quantities are generated through a fixed-point equation as follows.

	For all $\mu^G,$ set $\tilde{\gamma} = \theta[z]$. Then $(\tilde{\gamma},V)$ are solution of the following fixed-point equation\footnote{We discuss the existence of solution of this fixed-point equation in Section~\ref{sec:Existence}}, $\forall z\in\cZ,x^{\alpha}\in \cX$,
	\begin{align}
		\label{eq:m_FP_ih}
		\tilde{\gamma}(\cdot|x^{\alpha}) \in \arg\max_{\gamma(\cdot|x^{\alpha})}&\E^{\gamma(\cdot|x^{\alpha})} [R(x^{\alpha},A^{\alpha},\mu^G;g^{\alpha})+\nn\\
		&\delta V(\phi(z,\tgamma), X^{{\alpha}'};g^{\alpha}) | \mu^G,x^{\alpha}] ,
	\end{align}		
	\begin{align}
		V(z,x^{\alpha}) =\  &\E^{\tilde{\gamma}(\cdot|x^{\alpha})} [ R(x^{\alpha},A^{\alpha},\mu^G;g^{\alpha})+\nn\\
		&\delta V (\phi(\mu^G,\tgamma;g^{\alpha}), X^{{\alpha}'})\vert \mu^G,x^{\alpha}]. 
	\end{align}
	where expectation in \eqref{eq:m_FP_ih} is with respect to random variable $(A^{\alpha},X^{{\alpha},\prime})$ through the measure $\gamma(a^{\alpha}|x^{\alpha})Q^{\alpha}(x^{{\alpha}'}|x^{\alpha},a^{\alpha},\mu^G)$.

	Then an equilibrium strategy is defined as 
	\begin{align}
		\tilde{\sigma}^{\alpha}(a_t^{\alpha}|\mu^G_{1:t},x_{1:t}^{\alpha}) = \tilde{\gamma}(a_t^{\alpha}|x_t^{\alpha}), \label{eq:sigma_ih}
	\end{align}
	where $\tilde{\gamma} = \theta[\mu^G_t]$.

	The following theorem shows that the strategy thus constructed is a \gmfe of the game.

	\begin{theorem}
	\label{thih}
		A strategy $(\tsigma)$ constructed from the above algorithm is a \gmfe of the game i.e. $\forall t, h^{\alpha}_t \in \cH^{\alpha}_t, {\sigma^{\alpha}}$,

		\begin{align}
			\label{eq:prop_ih}
			&\E^{(\tsigma^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^\infty \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right] \geq\nn\\
			&\E^{({\sigma}^{\alpha} \tsigma^{-\alpha})}\left[\sum_{n=t}^\infty \delta^{n-t} R(X_n^{\alpha},A_n^{\alpha},\mu^G_n;g^{\alpha})|\mu^G_{1:t},x_{1:t}^{\alpha}\right], 
		\end{align} 
	\end{theorem}
	\begin{proof}
		Please refer to the online version for proofs.
	\end{proof}

\subsection{Converse}
	In the following, we show that every \gmfe can be found using the above backward recursion.
	\begin{theorem}[Converse]
	\label{thm:2ih}
		Let $\tsigma$ be a \gmfe the graphon mean field game. Then there exists an equilibrium generating function $\theta$	that satisfies \eqref{eq:m_FP} in backward recursion such that  $\tsigma$ is defined using $\theta$.
	\end{theorem}
	\begin{proof}
		Please refer to the online version for the proofs.
	\end{proof}

\subsection{Backward recursive algorithm for \gmft}

In this subsection, we will provide a methodology to generate optimal control policy for coupled teams with mean field sharing. We define an optimal policy $(\theta_t)_{t\in[T]}$, where $\theta_t:\cZ\to\times_{\alpha\in[0,1]}\{\cX^\alpha\to\mathcal{P}(\cA^\alpha) \}^\alpha$, where for each $\mu^G_t $, we generate $\tgamma_t = \theta_t[\mu^G_t]$ and $\tgamma_t = (\tgamma^\alpha_t)_{\alpha\in[0,1]}$. In addition, we generate a reward-to-go function $(V_t)_{t\in[T]}$, where $V_t:\cZ\to\mathbb{R}$. These quantities are generated as follows.
	\begin{enumerate}
		\item Initialize $\forall \mu^G_{T+1}\in \cX$,
		\begin{align}
			V_{T+1}(\mu^G_{T+1}) \defeq 0.   \label{eq:VT1+1}
		\end{align}

		\item For $t = T,T-1, \ldots 1, \ \forall \mu^G_t$, let $\theta_t[\mu^G_t] $ be generated as follows. Set $\tilde{\gamma}_t = \theta_t[\mu^G_t]$, where $\tilde{\gamma}_t$. $\forall i \in [N]$,
		\begin{align}
				\tilde{\gamma}_t \in  &\arg\max_{\gamma_t} \E^{\gamma_t,\mu_t^G}[ R_c(A_t,\mu^G_t;g)+\nn\\
				&\delta V_{t+1}(\phi(\mu^G_t,\gamma_t;g)) | \mu^G_t] , \label{eq:m_FP1}
		\end{align}
		where expectation in \eqref{eq:m_FP1} is with respect to random variable $(A_t)$ through the probability measure $\left(\gamma_t^\alpha\left(a^\alpha_t\vert x_t^\alpha\right)\mu^\alpha_t\left(x_t^\alpha\right)\right)_{\alpha\in[0,1]}$.

		Furthermore, using the quantity $\tilde{\gamma}_t$ found above, define
		\begin{align}
			V_{t}(\mu^G_t)&\defeq\E^{\tilde{\gamma}_t, \mu^G_t}[R_c(A_t,\mu^G_t;g)+\nn\\
			&\delta V_{t+1}(\phi(\mu^G_t,\tgamma_t)) | \mu^G_t].  \label{eq:Vdef1}
		\end{align}
	\end{enumerate}
	Then, an optimlal strategy is defined as 
	\begin{align}
		\tilde{\sigma}_t(a_t|\mu^G_{1:t}) = \tilde{\gamma}_t, \label{eq:sigma_fh1}
	\end{align}
	where $\tilde{\gamma}_t = \theta[\mu^G_t]$. 
	The following theorem shows that the strategy thus constructed is optimal.
	\begin{theorem}
	\label{thih1}
		A strategy $(\tsigma)$ constructed from the above algorithm is team optimal i.e. $\forall t, h_t \in \cH_t, {\sigma}$,

		\begin{align}
			\label{eq:prop_ih1}
			&\E^{\tsigma}\left[\sum_{n=t}^\infty \delta^{n-t} R_c(A_n,\mu^G_n;g)|\mu^G_{1:t}\right] \geq\nn\\
			&\E^{({\sigma} \tsigma)}\left[\sum_{n=t}^\infty \delta^{n-t} R(X_n,A_n,\mu^G_n;g)|\mu^G_{1:t}\right], 
		\end{align} 
	\end{theorem}
	\begin{proof}
		Please refer to the online version for proofs.
	\end{proof}
